Calliope: Automatic Visual Data Story Generation from a Spreadsheet

Visual data stories shown in the form of narrative visualizations such as a poster or a data video, are frequently used in data-oriented storytelling to facilitate the understanding and memorization of the story content. Although useful, technique barriers, such as data analysis, visualization, and scripting, make the generation of a visual data story difficult. Existing authoring tools rely on users' skills and experiences, which are usually inefficient and still difficult. In this paper, we introduce a novel visual data story generating system, Calliope, which creates visual data stories from an input spreadsheet through an automatic process and facilities the easy revision of the generated story based on an online story editor. Particularly, Calliope incorporates a new logic-oriented Monte Carlo tree search algorithm that explores the data space given by the input spreadsheet to progressively generate story pieces (i.e., data facts) and organize them in a logical order. The importance of data facts is measured based on information theory, and each data fact is visualized in a chart and captioned by an automatically generated description. We evaluate the proposed technique through three example stories, two controlled experiments, and a series of interviews with 10 domain experts. Our evaluation shows that Calliope is beneficial to efficient visual data story generation.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections-back/4-2-algorithm.tex <==
\subsection{Story Generation Algorithm}
In \name, we introduce an intelligent algorithm that generates data facts from an input spreadsheet and threads them in logic to create a meaningful data story. However design such an algorithm is quite challenge. The story design space, formulated by a collection of data facts generated from the input spreadsheet, could be extremely large due to the huge number of possible combinations of the fact fields event based on a small dataset. It is almost impossible for the algorithm to generate all facts first and then pick up those important ones to build the story as users cannot afford a long waiting time ({\bf R2}). We addressed this issue by introducing an efficient logic-oriented searching algorithm based on the Monte Carlo tree search~\cite{browne2012survey,silver2016mastering}. It can efficiently explore a large space that contains numerous status via a searching process organized by a tree structure and guided by a reward function.

Algorithm~\ref{alg:generation} provides an overview of the proposed technique. It takes a spreadsheet $\mathcal{D}$, the desired story length $\mathcal{L}$, and a set of parameters \{$w_d, w_i, w_l$\} as the inputs and outputs a story  $\mathcal{S} = \{f_1,\cdots,f_n\}$. Here, the parameters are given by users that indicate their personal preferences of the generated story in terms of its fact diversity ($w_d$), the data coverage rate ($w_d$), and logicality ($w_l$). Specifically, the algorithm first generates a set of initial facts in three fact types, i.e., value, trend, and categorization, that are most frequently used as the starting points in a data story according to our preliminary survey as shown in Fig.~\ref{fig:statistic}(b). The most important one is selected as the initial fact in $\mathcal{S}$, denoted as $f_0$, and used as the root of a search tree. In the next, the algorithm expands $f_0$ in the tree by creating a set of data facts as its children that are logically relevant to $f_0$. 

which is estimated by as reward function  estimated by a reward function,  

based on which the  a search tree is gradually generated. 

%The while loop on \textbf{line 3} guarantee the story should reach the defined length. \textbf{Line 4} to \textbf{8} is the general MCTS approach, which should be limited in the computational time. In each iteration, the strategy determines an action $(f_l,r_l)$ given a story state $S$ (\textbf{line 5}), where $f_l$ and $r_l$ is the last fact and relation that can be reached according to the tree policy (Section \ref{4.2.1}). After take the action $(f_l,r_l)$, \textbf{line 6} runs a random simulation from the current state of story to the terminal. The $reward$ for terminal $S$ can be calculated according to our reward function (Section \ref{4.2.2}). The back-propagation will update the reward scores and visitation frequencies on the search tree in \textbf{line 7}. As the result of the overall search, BestChild($S$) is the next fact and relation that leads story to the best reward. So we take the result as next action to append the current $S$ in \textbf{line 9}. After reach the maximum of the story length, we can get the final generated $S$. Moreover, in \textbf{line 11} we aggregate $S$ to make it more concise using the method mentioned in Section \ref{4.3}.

\begin{algorithm}[htb]
    \label{alg:generation}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$data$}
    \Output{$S$}
    % \KwResult{Write here the result }
    $f_0$ $\leftarrow$ InitalFact($data$)\;
    $S$ $\leftarrow$ [$f_0$]\;
    \While{length(S) \textless max}{
        \While{within computational time}{
            ($f_l$,$r_l$) $\leftarrow$ TreePolicy($S$)\;
            $reward$ $\leftarrow$ DefaultPolicy($story(f_l, r_l)$)\;
            Backpropagation(($f_l$,$r_l$), $reward$)\;
        }
        $S$.insert(BestChild($S$))\;
    }
    $S$ $\leftarrow$ Aggregation($S$)\;
    \Return $S$\;
    \caption{Data Story Generation}
\end{algorithm}

\subsubsection{Logic Calculation}

% Describing how did we ensures the story logic and reduce the search space. Describe the statistics that we summarized based on the preliminary survey.

A $tree$ $policy$ determines the most possible node to reach in each iteration of MCTS. In data story generation, the $tree policy$ is used to find the next fact to expand the story. To ensure the facts in story are meaningful connected and reduce the search space, we introduce coherence relations as the latent relation between the adjacent facts to guide a logic-oriented tree policy in MCTS. In the discourse, coherence relations refers to informational relations that hold between natural language sentences \cite{hobbs1985coherence}. According to preliminary data videos survey and related corpus studies \cite{wolf2005representing, wellner2006classification}, we summarize 6 discourse relations in data stories in Table \ref{table:relation}. A pair of facts can be described by three components $(f_a, r_{ab}, f_b)$, where $f_a$ and $f_b$ denote two adjacent facts connected by relation $r_{ab}$.

\input{tables/4-relation}

A $tree$ $policy$ determines the most possible node to reach in each iteration of MCTS. In data story generation, the $tree policy$ is used to find the next fact to expand the story. To ensure the facts in story are meaningful connected and reduce the search space, we introduce coherence relations as the latent relation between the adjacent facts to guide a logic-oriented tree policy in MCTS. In the discourse, coherence relations refers to informational relations that hold between natural language sentences \cite{hobbs1985coherence}. According to preliminary data videos survey and related corpus studies \cite{wolf2005representing, wellner2006classification}, we summarize 6 discourse relations in data stories in Table \ref{table:relation}. A pair of facts can be described by three components $(f_a, r_{ab}, f_b)$, where $f_a$ and $f_b$ denote two adjacent facts connected by relation $r_{ab}$.

\input{tables/4-relation}

We regard these relations as the constraints in tree policy. \name applies the rules in the defined relations to keep the connection between $f_a$ and $f_b$. As follow, when the current fact is $f_a$ and relation is $r_{ab}$, the next fact $f_b$ can be derived after a set of edit operations from $f_a$:

\begin{itemize}
    \item {\bf Similarity} modifies ($meausre$/$breakdown$/categorical filter in $subspace$) in $f_a$ to construct the $f_b$. It juxtaposes two facts with same measurement or same scope of data, such as ``the confirmed count of COVID-19 in different provinces".
    \item {\bf Temporal} adds/removes/modifies the temporal filter of $subspace$ in $f_a$ to construct the $f_b$. It statement two facts based on time, such as ``the confirmed count of COVID-19 in February and March".
    \item {\bf Contrast} modifies ($meausre$/filter in $subspace$) in $f_a$. In addition, the result should be the opposite fact to $f_a$, thus we take it as $f_b$. In this relation, $f_a$ and $f_b$ are reverse to each other, such as ``the decreasing trend of new confirmed count of COVID-19 in China and the increasing trend in other countries". 
    \item {\bf Causality} modifies $meausre$ that has the cause-effect relation to the $f_a$. $f_b$ should be the reason of $f_a$, such as ``the confirmed count leads to the death count of COVID-19". The causality discover technique can be used to build a causal graph for the multi-dimensional data \cite{schaechtle2013multi}. The directed link in the causal graph means the causal relation from one numerical data to another. Thus we use the causal graph to modify the $measure$.
    \item {\bf Elaboration} add filter in $subspace$ or add $focus$ from $f_a$ to $f_b$.  It means $f_b$ is the specific condition to $f_a$, such as ``the confirmed count of COVID-19 in China and details in each provinces".
    \item {\bf Generalization} remove filter in $subspace$ or remove $focus$ from $f_a$ to $f_b$. It means $f_b$ is the general condition to $f_a$, such as ``the confirmed count of COVID-19 in China and overall information in the world".
\end{itemize}

In addition, we follow the statistic of narrative logic frequently used behind each fact type (Table~\ref{tab:logic}) to determine the probability of each relation during tree search. 

\label{4.2.1}

\subsubsection{Reward Function}
% Describing the reward function followed by the details of each terms in the function. The key is to clearly describe the design rationale of each term.

The reward function is to ensure the quality of the story generation. As we mentioned before, our system should generate a meaningful story in a clear logic with correct data. The meaningful story refers to a data story with a high importance score, which can be measured by the information entropy and significance.

Besides the story importance, the story should also provide the narrative logic, and believable content. Furthermore, the content in story should should be diverse to avoid a boring presentation. Therefore, the final reward of story also consider narrative logic, data integrity, and diversity. We put these three parameters into the coefficient of preference which can be adjusted by the user.

The total reward of story is the product of the coefficient of user preference and the importance score of the story. Bringing each parameters together, the final $reward$ is:

\begin{equation}
reward =  (\alpha \cdot Diversity  + \beta \cdot Integrity + \gamma \cdot Logicality) \cdot score(S)
\end{equation}
where $\alpha$, $\beta$ and $\gamma$ is the weight in [0,1] and the sum of them is equal to 1. Users can determine the value by interaction in the storyline view. The interaction detail will be introduced in Section~\ref{5.4}.

Based on the information theory, we define the information entropy of story $S$ as $H(S)$ by the formula of information entropy:

\begin{equation}
    H(S)=-\sum_{i=1}^{m} P(f_i) \log _{2}\left(P(f_i)\right) = \sum_{i=1}^{n} { P(f_i) \cdot I(f_i) }
\end{equation}

We add significance importance of each fact into this formula to calculate the importance score of the story $score(S)$. Then, we put formula of fact importance into $score(S)$.

\begin{equation}
score(S) = \sum_{i=1}^{n} { P(f_i) \cdot S(f_i) \cdot I(f_i) } = \sum_{i=1}^{n} { P(f_i) \cdot score(f_i) }
\end{equation}

\textbf{Logicality} represents the logic of the story.
In the logic tree search, we only consider the logic from current fact to next relation. By contrast, we consider the logic from fact to last relation in reward term. Logicality is the average of each conditional probability of last relation $r_{i-1}$ given fact $f_{i}$:

\begin{equation}
Logicality = \frac{1}{n-1}\sum_{i=1}^{n-1}P\left(r_{i-1} | f_{i}\right)
\end{equation}

\textbf{Diversity} represents the diversity of the story.
When there are more various fact types in a story, the story is considered more diverse. We define $m$ as the number of fact types in the story and ${p}_{j}$ as the proportion of $j$th fact type in the story. The diversity is calculated as the follow, where the former item is to make sure more unique fact types in the story and the latter item is the normalized Shannon diversity index to keep these fact types have roughly equal proportion:

\begin{equation}
Diversity = \frac{m}{\max(n,10)} \cdot -\frac{\sum_{j=1}^{m} {p}_{j} \cdot \ln \left({p}_{j}\right)}{\ln (m)} 
\end{equation}

\textbf{Integrity} represents the data integrity of the story.
The more complete the story cover the spreadsheet, the better the data integrity. The calculation method is to take the union of the table cells covered by each fact and divide by the count of total table cells:

\begin{equation}
Integrity = \frac{count_{cell}(\bigcup\limits_{i=0}^{n-1} f_{i})}{count_{cell}(data)}
\end{equation}

\label{4.2.2}

\subsection{Story Aggregation}
% Describe the fact clustering algorithm, especially the distance measure and features that we used to calculate the distance. Describe the fact aggregation rule (the big table). Discuss the potential issues such as the perception cost. 

For now, the story pieces in our generated data story only convey single fact. However, the compound fact is the common used fact that consists of multiple primitive facts \cite{amar2005low, chen2009toward}. For instance, "The trend of sales is decreasing and the maximum of sales is in 2007" is a compound fact that involves a trend fact and an extreme fact. To keep the story concise, \name provides an option for users to aggregate the story by merging single facts into a compound one automatically.

The story aggregation process consists of three major steps: (1) similarity measuring, (2) hierarchical clustering, and (3) fact merging.

First, we measures the similarity between data facts using the overlap similarity for categorical data \cite{boriah2008similarity}. The overlap similarity of the $type$ is 0 when types of two facts are no match, and 1 when the attribute values match. For the $measure$ and the $breakdown$, the similarity is the proportion of the fields in common. For the $subspace$ and the $focus$, we use the the fraction of union covered by intersection for similarity calculation. The similarity in total is the sum of these five results.

Then, we aggregate the data facts into a hierarchical structure based on the similarity using hierarchical clustering technique. After clustering, the pairs of leaf nodes, such as the dashed box in fig, are the potential facts to be merged. These pairs of facts are ranked according to the similarity.The more similar facts have more tendency to be merged.\name provides a slider bar that allows users to control the level of story aggregation in percentage, with a value of 0\% to present single facts, and a value of 100\% to merge all pairs of data facts.

To present the compound fact, \name merge facts in two aspects, including visualization and natural language. For simplicity, we define a rule table for each combinations of two fact types. In the table, we choose chart type for compound fact according to the intersection of chart candidates for each primitive fact type. We also merge the fact tuples that have no conflict between each other. If there is no common chart type between two facts or conflict in the fact tuples, we simply place the two visualization by juxtaposition. For example, there is a trend fact and a extreme fact share same $measure$, $subspace$, and $breakdown$ shown in Fig.\ref{fig:aggregation}. The difference is that the extreme fact has an additional \textit{focus} which highlight the maximum value. Based on our rule table, both of these two facts can use the line chart to present the information. As a result, the compound fact use line chart  which is shown in Fig.\ref{fig:aggregation}. For the description of compound fact, we choose to join together two sentences from both primitive facts.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/aggregation.png}
    \caption{Compound fact} 
    \label{fig:aggregation}
\end{figure}

Up to this point, \name does not consider the perception cost during the fact merging \cite{hullman2013deeper}. Besides, the natural language in the compound fact may has redundancy, which can be solved by NLP techniques such as coreference resolution \cite{ng2002improving}. We leave these questions in the future work.

\label{4.3}

% \subsection{Story Generation Algorithm}
% % First describe the algorithm overview via pseudocode and explain the algorithm pipeline by important steps.

% In our definition, data story $S$ consists of a sequence of data facts $\{f_1, f_2, \cdots, f_n\}$. The fundamental story generation approach is to pick and organize the data facts by exploring the multi-dimensional space of the spreadsheet. However, when the dimensionality of data increases, the space of fact will increase exponentially. Thus, the generation can be defined as a search problem in the data space. Toward avoid the curse of dimensionality, The Monte Carlo tree search (MCTS) \cite{browne2012survey} is a promising solution in large search space. It has a successful case in the game with large search space, like GO \cite{silver2016mastering}. Since MCTS doesn't necessarily require domain knowledge, we borrow this idea into data story generation.

% The story generation algorithm is summarized in pseudocode in Algorithm \ref{alg:generation}. The input of algorithm is data from spreadsheet and the out put is a story. \textbf{Line 1} and \textbf{2} of the algorithm is the story initialization. Here $f_0$ is the initial fact in the story $S$ and the root node in the tree. We limit the search space of the start point $f_0$ within top 3 fact types based on the Fig.~\ref{fig:fact-relation-rank}. The while loop on \textbf{line 3} guarantee the story should reach the defined length. \textbf{Line 4} to \textbf{8} is the general MCTS approach, which should be limited in the computational time. In each iteration, the strategy determines an action $(f_l,r_l)$ given a story state $S$ (\textbf{line 5}), where $f_l$ and $r_l$ is the last fact and relation that can be reached according to the tree policy (Section \ref{4.2.1}). After take the action $(f_l,r_l)$, \textbf{line 6} runs a random simulation from the current state of story to the terminal. The $reward$ for terminal $S$ can be calculated according to our reward function (Section \ref{4.2.2}). The back-propagation will update the reward scores and visitation frequencies on the search tree in \textbf{line 7}. As the result of the overall search, BestChild($S$) is the next fact and relation that leads story to the best reward. So we take the result as next action to append the current $S$ in \textbf{line 9}. After reach the maximum of the story length, we can get the final generated $S$. Moreover, in \textbf{line 11} we aggregate $S$ to make it more concise using the method mentioned in Section \ref{4.3}.

% \begin{algorithm}[htb]
%     \label{alg:generation}
%     \SetAlgoLined
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$data$}
%     \Output{$S$}
%     % \KwResult{Write here the result }
%     $f_0$ $\leftarrow$ InitalFact($data$)\;
%     $S$ $\leftarrow$ [$f_0$]\;
%     \While{length(S) \textless max}{
%         \While{within computational time}{
%             ($f_l$,$r_l$) $\leftarrow$ TreePolicy($S$)\;
%             $reward$ $\leftarrow$ DefaultPolicy($story(f_l, r_l)$)\;
%             Backpropagation(($f_l$,$r_l$), $reward$)\;
%         }
%         $S$.insert(BestChild($S$))\;
%     }
%     $S$ $\leftarrow$ Aggregation($S$)\;
%     \Return $S$\;
%     \caption{Data Story Generation}
% \end{algorithm}

% \subsubsection{Logic Calculation}

% % Describing how did we ensures the story logic and reduce the search space. Describe the statistics that we summarized based on the preliminary survey.

% A $tree$ $policy$ determines the most possible node to reach in each iteration of MCTS. In data story generation, the $tree policy$ is used to find the next fact to expand the story. To ensure the facts in story are meaningful connected and reduce the search space, we introduce coherence relations as the latent relation between the adjacent facts to guide a logic-oriented tree policy in MCTS. In the discourse, coherence relations refers to informational relations that hold between natural language sentences \cite{hobbs1985coherence}. According to preliminary data videos survey and related corpus studies \cite{wolf2005representing, wellner2006classification}, we summarize 6 discourse relations in data stories in Table \ref{table:relation}. A pair of facts can be described by three components $(f_a, r_{ab}, f_b)$, where $f_a$ and $f_b$ denote two adjacent facts connected by relation $r_{ab}$.

% \input{tables/4-relation}

% We regard these relations as the constraints in tree policy. \name applies the rules in the defined relations to keep the connection between $f_a$ and $f_b$. As follow, when the current fact is $f_a$ and relation is $r_{ab}$, the next fact $f_b$ can be derived after a set of edit operations from $f_a$:

% \begin{itemize}
%     \item {\bf Similarity} modifies ($meausre$/$breakdown$/categorical filter in $subspace$) in $f_a$ to construct the $f_b$. It juxtaposes two facts with same measurement or same scope of data, such as ``the confirmed count of COVID-19 in different provinces".
%     \item {\bf Temporal} adds/removes/modifies the temporal filter of $subspace$ in $f_a$ to construct the $f_b$. It statement two facts based on time, such as ``the confirmed count of COVID-19 in February and March".
%     \item {\bf Contrast} modifies ($meausre$/filter in $subspace$) in $f_a$. In addition, the result should be the opposite fact to $f_a$, thus we take it as $f_b$. In this relation, $f_a$ and $f_b$ are reverse to each other, such as ``the decreasing trend of new confirmed count of COVID-19 in China and the increasing trend in other countries". 
%     \item {\bf Causality} modifies $meausre$ that has the cause-effect relation to the $f_a$. $f_b$ should be the reason of $f_a$, such as ``the confirmed count leads to the death count of COVID-19". The causality discover technique can be used to build a causal graph for the multi-dimensional data \cite{schaechtle2013multi}. The directed link in the causal graph means the causal relation from one numerical data to another. Thus we use the causal graph to modify the $measure$.
%     \item {\bf Elaboration} add filter in $subspace$ or add $focus$ from $f_a$ to $f_b$.  It means $f_b$ is the specific condition to $f_a$, such as ``the confirmed count of COVID-19 in China and details in each provinces".
%     \item {\bf Generalization} remove filter in $subspace$ or remove $focus$ from $f_a$ to $f_b$. It means $f_b$ is the general condition to $f_a$, such as ``the confirmed count of COVID-19 in China and overall information in the world".
% \end{itemize}

% In addition, we follow the statistic of narrative logic frequently used behind each fact type (Table~\ref{tab:logic}) to determine the probability of each relation during tree search. 

% \label{4.2.1}

% \subsubsection{Reward Function}
% % Describing the reward function followed by the details of each terms in the function. The key is to clearly describe the design rationale of each term.

% The reward function is to ensure the quality of the story generation. As we mentioned before, our system should generate a meaningful story in a clear logic with correct data. The meaningful story refers to a data story with a high importance score, which can be measured by the information entropy and significance.

% Besides the story importance, the story should also provide the narrative logic, and believable content. Furthermore, the content in story should should be diverse to avoid a boring presentation. Therefore, the final reward of story also consider narrative logic, data integrity, and diversity. We put these three parameters into the coefficient of preference which can be adjusted by the user.

% The total reward of story is the product of the coefficient of user preference and the importance score of the story. Bringing each parameters together, the final $reward$ is:

% \begin{equation}
% reward =  (\alpha \cdot Diversity  + \beta \cdot Integrity + \gamma \cdot Logicality) \cdot score(S)
% \end{equation}
% where $\alpha$, $\beta$ and $\gamma$ is the weight in [0,1] and the sum of them is equal to 1. Users can determine the value by interaction in the storyline view. The interaction detail will be introduced in Section~\ref{5.4}.

% Based on the information theory, we define the information entropy of story $S$ as $H(S)$ by the formula of information entropy:

% \begin{equation}
%     H(S)=-\sum_{i=1}^{m} P(f_i) \log _{2}\left(P(f_i)\right) = \sum_{i=1}^{n} { P(f_i) \cdot I(f_i) }
% \end{equation}

% We add significance importance of each fact into this formula to calculate the importance score of the story $score(S)$. Then, we put formula of fact importance into $score(S)$.

% \begin{equation}
% score(S) = \sum_{i=1}^{n} { P(f_i) \cdot S(f_i) \cdot I(f_i) } = \sum_{i=1}^{n} { P(f_i) \cdot score(f_i) }
% \end{equation}

% \textbf{Logicality} represents the logic of the story.
% In the logic tree search, we only consider the logic from current fact to next relation. By contrast, we consider the logic from fact to last relation in reward term. Logicality is the average of each conditional probability of last relation $r_{i-1}$ given fact $f_{i}$:

% \begin{equation}
% Logicality = \frac{1}{n-1}\sum_{i=1}^{n-1}P\left(r_{i-1} | f_{i}\right)
% \end{equation}

% \textbf{Diversity} represents the diversity of the story.
% When there are more various fact types in a story, the story is considered more diverse. We define $m$ as the number of fact types in the story and ${p}_{j}$ as the proportion of $j$th fact type in the story. The diversity is calculated as the follow, where the former item is to make sure more unique fact types in the story and the latter item is the normalized Shannon diversity index to keep these fact types have roughly equal proportion:

% \begin{equation}
% Diversity = \frac{m}{\max(n,10)} \cdot -\frac{\sum_{j=1}^{m} {p}_{j} \cdot \ln \left({p}_{j}\right)}{\ln (m)} 
% \end{equation}

% \textbf{Integrity} represents the data integrity of the story.
% The more complete the story cover the spreadsheet, the better the data integrity. The calculation method is to take the union of the table cells covered by each fact and divide by the count of total table cells:

% \begin{equation}
% Integrity = \frac{count_{cell}(\bigcup\limits_{i=0}^{n-1} f_{i})}{count_{cell}(data)}
% \end{equation}

% \label{4.2.2}

% \subsection{Story Aggregation}
% % Describe the fact clustering algorithm, especially the distance measure and features that we used to calculate the distance. Describe the fact aggregation rule (the big table). Discuss the potential issues such as the perception cost. 

% For now, the story pieces in our generated data story only convey single fact. However, the compound fact is the common used fact that consists of multiple primitive facts \cite{amar2005low, chen2009toward}. For instance, "The trend of sales is decreasing and the maximum of sales is in 2007" is a compound fact that involves a trend fact and an extreme fact. To keep the story concise, \name provides an option for users to aggregate the story by merging single facts into a compound one automatically.

% The story aggregation process consists of three major steps: (1) similarity measuring, (2) hierarchical clustering, and (3) fact merging.

% First, we measures the similarity between data facts using the overlap similarity for categorical data \cite{boriah2008similarity}. The overlap similarity of the $type$ is 0 when types of two facts are no match, and 1 when the attribute values match. For the $measure$ and the $breakdown$, the similarity is the proportion of the fields in common. For the $subspace$ and the $focus$, we use the the fraction of union covered by intersection for similarity calculation. The similarity in total is the sum of these five results.

% Then, we aggregate the data facts into a hierarchical structure based on the similarity using hierarchical clustering technique. After clustering, the pairs of leaf nodes, such as the dashed box in fig, are the potential facts to be merged. These pairs of facts are ranked according to the similarity.The more similar facts have more tendency to be merged.\name provides a slider bar that allows users to control the level of story aggregation in percentage, with a value of 0\% to present single facts, and a value of 100\% to merge all pairs of data facts.

% To present the compound fact, \name merge facts in two aspects, including visualization and natural language. For simplicity, we define a rule table for each combinations of two fact types. In the table, we choose chart type for compound fact according to the intersection of chart candidates for each primitive fact type. We also merge the fact tuples that have no conflict between each other. If there is no common chart type between two facts or conflict in the fact tuples, we simply place the two visualization by juxtaposition. For example, there is a trend fact and a extreme fact share same $measure$, $subspace$, and $breakdown$ shown in Fig.\ref{fig:aggregation}. The difference is that the extreme fact has an additional \textit{focus} which highlight the maximum value. Based on our rule table, both of these two facts can use the line chart to present the information. As a result, the compound fact use line chart  which is shown in Fig.\ref{fig:aggregation}. For the description of compound fact, we choose to join together two sentences from both primitive facts.

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=\linewidth]{figures/aggregation.png}
%     \caption{Compound fact} 
%     \label{fig:aggregation}
% \end{figure}

% Up to this point, \name does not consider the perception cost during the fact merging \cite{hullman2013deeper}. Besides, the natural language in the compound fact may has redundancy, which can be solved by NLP techniques such as coreference resolution \cite{ng2002improving}. We leave these questions in the future work.

% \label{4.3}

==> sections-back/4-datafacts.tex <==
\section{Story Generation Engine}
\label{sec:engine}
In this section, we describe the technique details of the visual data story generation engine introduced in \name. Before describing the algorithm, we first introduce different types of data facts and their importance measures. 

\subsection{Data Facts}
Data facts are the elementary pieces that build up a data story. In \name, we formally define fact as a 5-tuple 

Based on preliminary study and formative work \cite{wang2019datashot}, Calliope provides a formal model for representing data facts.
In our definition, a data fact consist of a five-tuple, including \textit{type}, \textit{measure}, \textit{subspace}, \textit{group-by} and \textit{focus}.
$$
fact := (type, measure, subspace, groupby, focus)
$$

The \textit{type} definition identifies the fact type from 10 pre-defined taxonomies, including \textit{value}, \textit{difference}, \textit{proportion}, \textit{trend}, \textit{categorization}, \textit{distribution}, \textit{rank}, \textit{association}, \textit{extreme} and \textit{outlier}.
These 10 types derive from our preliminary survey on data videos and several formative works \cite{wang2019datashot, chen2009toward}. 
The \textit{measure} determines which numerical field and aggregation function to use as the measurement in the fact.
The \textit{subspace} specifies the range of data that fulfill a filter condition.
The \textit{group-by} groups records that have same value in categorical or temporal fields into summary records.
The \textit{focus} highlights the specific information in the subspace.

Table \ref{tab:fact_table} summarizes the rules to construct the data fact for each fact type.
As shown in the table, \textit{measure}, \textit{group-by} and \textit{focus} are not necessary for all fact types.
The definition of each fact type are depicted in the following list.
To explain the meaning of each fact type, we use a sample spreadsheet about automatic sales.
The columns' information is shown in Table \ref{table:tabledetail}.

\begin{table}[htb]
    \label{table:tabledetail}
    \caption{The information of columns in the sample}
    \centering
    \small
    \begin{tabular}{ccl}
    \hline
    field name & type & description \\ \hline
    Sales & numerical & automobile sales \\ 
    Income & numerical & automobile income \\ 
    Category & categorical & types of automobile (e.g. SUV, Compact) \\ 
    Brand & categorical & brands of automobile (e.g. BMW, Ford) \\ 
    Year & temporal & year of Sales (2007-2011) \\ \hline
    \end{tabular}
\end{table}

\begin{itemize}

    \item \textbf{Value} is defined on (\textit{measure}, \textit{subspace}).
    It derives the value according to the \textit{measure} in \textit{subspace}. 
    E.g. Show total sales in Brand Ford.
    
    \item \textbf{Difference} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It compares the \textit{measure} of two \textit{focus} on \textit{group-by} in \textit{subspace}.
    E.g. Compare difference between sales of SUV and Compact in Brand BMW.
    
    \item \textbf{Proportion} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It shows the proportion of the \textit{measure} in the \textit{focus} from all \textit{group-by}s in \textit{subspace}.
    E.g. Show proportion of SUV in total sales of Brand Ford.
    
    \item \textbf{Trend} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}).
    It shows the \textit{measure} order by the temporal \textit{group-by} in \textit{subspace}.
    E.g. Show the trend of sales in Brand Ford order by year.
    
    \item \textbf{Categorization} is defined on (\textit{subspace}, \textit{group-by}).
    It lists all \textit{group-by}s in \textit{subspace}.
    E.g. Show all categories contained in Brand Ford.
    
    \item \textbf{Distribution} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}).
    It shows the \textit{measure} of each \textit{group-by} in \textit{subspace}. 
    E.g. Show the sales of each category in Brand Ford.
    
    \item \textbf{Rank} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It lists all \textit{group-by} order by \textit{measure} in \textit{subspace} and \textit{focus} on the top rank.
    E.g. List the sales rank of brand in 2011.
    
    \item \textbf{Association} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}).
    It shows the relation between two \textit{measure}s by \textit{group-by} in \textit{subspace}.
    E.g. Show the relationship between sales and income in each brand in 2011.
    
    \item \textbf{Extreme} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It shows the \textit{measure} of each \textit{group-by} in \textit{subspace} and \textit{focus} on the extreme.
    E.g. Show the best-selling category in Brand Ford.
    
    \item \textbf{Outlier} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It shows the \textit{measure} of each \textit{group-by} in \textit{subspace} and \textit{focus} on the outlier.
    E.g. Show the outlier of sales by year in Brand Ford.
    
\end{itemize}

According to this fact definition, We describe a single data fact using a JSON specification in Calliope.
Based on the automobile spreadsheet, we demonstrate a \textit{Proportion} fact in Listing \ref{lst:json}.
The \textit{measure} of the fact is total sum of ``Sales".
The \textit{subspace} is the records when ``Brand" is equal to ``Ford".
The \textit{group-by} divide the subspace by ``Category", and the \textit{focus} is the records when when ``Category" is equal to ``SUV".
The meaning of this specification is to show the proportion fact about total Sales of SUV in the Brand Ford.

\begin{lstlisting}[caption=JSON specification of a data fact,
basicstyle=\small, label={lst:json}, language=json,firstnumber=1]
{
    "type": "proportion",
    "measure": [{"field": "Sales", "aggregate": "sum"}],
    "subspace": [{"field": "Brand", "value": "Ford"}],
    "group-by": [{"field": "Category"}],
    "focus": [{"field": "Category", "value": "SUV"}]
}
\end{lstlisting}

In addition the basic fact defination, data facts also have \textit{parameter} to explain the status of the fact, such as increasing or decreasing in the \textit{trend} fact.
Table \ref{tab:fact_table} displays all \textit{parameter} in 10 fact types.
These \textit{parameter}s can be derived from the data and fact specification directly.
With the \textit{parameter}, we can generate natural language for each fact. 
The detail of facts to natural language will be descripted in Section 5.2.1.

\begin{table*}[t]
    \caption{Data Facts}
    \label{tab:fact_table}
    \small
    \def\arraystretch{1.2}
    \begin{tabular}{|l|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|l|p{7.7cm}|}
    \hline
    fact type & \multicolumn{1}{l|}{measure} & \multicolumn{1}{l|}{subspace} & \multicolumn{1}{l|}{group-by} & \multicolumn{1}{l|}{ focus } & parameter & sentence template \\ \hline
    Value & O & O & X & X & derived value & The \{\{aggregate\}\} \{\{measure\}\} is \{\{parameter\}\} when \{\{subspace\}\}. \\ \hline
    Difference & O & O & O & O & difference value & \begin{tabular}[c]{@{}l@{}}The difference between \{\{focus{[}1{]}\}\} and \{\{focus{[}2{]}\}\} regarding to their \\ \{\{aggregate\}\} \{\{measure\}\} is \{\{parameter\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Proportion & O & O & O & O & percentage & \begin{tabular}[c]{@{}l@{}}The \{\{focus\}\} accounts for \{\{parameter\}\} of the \{\{aggregate\}\} \\ \{\{measure\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Trend & O & O & O & X & increasing/decreasing & \begin{tabular}[c]{@{}l@{}}The trend of \{\{aggregate\}\} \{\{measure\}\} over \{\{group-by\}\} is \\ \{\{parameter\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Categorization & X & O & O & X & number of categories & \begin{tabular}[c]{@{}l@{}}Given \{\{subspace\}\}, there are \{\{parameter\}\} \{\{group-by\}\}(s) \\ which are \{\{C\_1\}\}, \{\{C\_2\}\}, \{\{...\}\}, and \{\{C\_n\}\}.\end{tabular} \\ \hline
    Distribution & O & O & O & X & N/A & \begin{tabular}[c]{@{}l@{}}The distribution of the \{\{aggregate\}\} \{\{measure\}\} over different \\ \{\{group-by\}\}(s) shows an overview of the data when \{\{subspace\}\}.\end{tabular} \\ \hline
    Rank & O & O & O & O & N/A & \begin{tabular}[c]{@{}l@{}}In the \{\{aggregate\}\} \{\{measure\}\} ranking of different \{\{group-by\}\}(s), \\ the top three \{\{group-by\}\}(s) are \{\{focus{[}0{]}\}\}, \{\{focus{[}1{]}\}, \{\{focus{[}2{]}\}\},\\ when \{\{subspace\}\}.\end{tabular} \\ \hline
    Association & O & O & O & X & correlation value & \begin{tabular}[c]{@{}l@{}}The Pearson correlation between the \{\{measure{[}1{]}\}\} and the \\ \{\{measure{[}2{]}\}\} is \{\{parameter\}\} in case of \{\{subspace\}\}.\end{tabular} \\ \hline
    Extreme & O & O & O & O & \begin{tabular}[c]{@{}l@{}}0: max/min\\ 1: extreme value\end{tabular} & \begin{tabular}[c]{@{}l@{}}Given \{\{subspace\}\}, the \{\{parameter{[}0{]}\}\} value of the \{\{aggregate\}\} \\ \{\{measure\}\}is \{\{parameter{[}1{]}\}\} when \{\{group-by\}\} is \{\{focus\}\}.\end{tabular} \\ \hline
    Outlier & O & O & O & O & outlier value & \begin{tabular}[c]{@{}l@{}}The\{\{aggregate\}\} \{\{measure\}\} of \{\{focus\}\} is an outlier when compare \\ with that of other \{\{group-by\}\}(s) when \{\{subspace\}\}.\end{tabular} \\ \hline
    \end{tabular}
\end{table*}

Calliope calculate the importance score $I(f)$ for a data fact $f$ to measure the value of fact.
The score contains two aspects: information importance ${\rm Info}(f)$ and significance importance ${\rm Sig}(f)$.
The importance score for each fact is:

\begin{equation}
    I(f) = {\rm Sig}(f) * {\rm Info}(f)
\end{equation}

\textbf{Information importance} is measured by Shannon entropy \cite{shannonentropy}, which is also called the self-information of a data fact.
The information importance should be high when an unlikely data fact is observed in spreadsheet.
It is calculated as follows, where $X$ is the scope of the data:

\begin{equation}
{\rm Info}(f) = -log_2(P(X))
\end{equation}

According our fact definition, the \textit{subspace} and the \textit{focus} are the only two elements that related to the scope of the data $X$.
So the probability of $X$ is then determined by the product of the probability of \textit{subspace} and conditional probability of \textit{focus} given \textit{subspace}:

\begin{equation}
P(X) = P(subspace) * P(focus | subspace)
\end{equation}

For now, we only support at most 2 fields in the subspace of the fact.
The following formulation is to calculate the probability of the subspace:

% \begin{equation}
% P(subspace)  =  P(field = K)
% \end{equation}
\begin{equation}
P(subspace)=\frac{1}{\sum_{i=0}^{2} C(n, i)}*\prod_{i=1}^{k}\frac{count({subspace}_i)}{count(all)}
\end{equation}
The former item is the probability of the occurence of the \textit{subspace}, where $n$ is the count of categorical and temporal fields in the spreadsheet, and $C(n,i)$ is the number of $i$-combinations from $n$ fields. 
The latter item is the probability of the \textit{subspace}, where $count({subspace}_i)$ is the count of records which fulfills the $i$th condition in \textit{subspace} and $count(all)$ is the total count of the spreadsheet.
When the \textit{subspace} includes two fields, we assume they are independent to each other.
So we calculate the product of the probabilities of two \textit{subspace}s.

The conditional probability of \textit{focus} given \textit{subspace} is determined by the fraction of the count of \textit{subspace} covered by the count of \textit{focus}:

\begin{equation}
P(focus|subspace)= \frac{count(focus)}{count(subspace)}
\end{equation}

\textbf{Significance importance} $Sig(f)$ is the measurement from the statistical aspect. 
To determine the importance of fact, significance is the weight for the information importance in [0, 1].
For instance, if a trend fact is steady with no obvious increasing or decreasing, it should have a low significance close to 0.
In contrast, a fact shows a clear rising trend line should get a high significance close to 1.
We calculate the significance importance of the fact using the methods in formative works \cite{ding2019quickinsights, tang2017extracting, wang2019datashot}.

\subsection{Story Generation Algorithm}
First describe the algorithm overview via pseudocode and explain the algorithm pipeline by important steps.

\subsubsection{Logic Calculation}
Describing how did we ensures the story logic and reduce the search space. Describe the statistics that we summarized based on the preliminary survey.

\subsubsection{Reward Function}
Describing the reward function followed by the details of each terms in the function. The key is to clearly describe the design rationale of each term.

We define the information entropy of the data story as $H(story)$.

\begin{equation}
H(story) = E(I(F)) = \sum_{i=1}^{n} { P(f_i) * I(f_i) }
\end{equation}
$I(f_i)$ is the quantity of information for the $i$th fact and the $X$ is the data of the fact.

Based on the information entropy, we add significance into the formulation to calculate the importance score of the story $I(story)$.

\begin{equation}
I(S)  = E(S(F) * I(F)) =  \sum_{i=1}^{n} { P(f_i) * S(f_i) * I(f_i) }
\end{equation}

The total story reward is the importance score of the story with the weight of user preference.

\begin{equation}
Reward = w_{S} * Importance(S)
\end{equation}

The weight of user preference includes: logicality, diversity and integrity.

\begin{equation}
w_{story} =  \alpha * Diversity  + \beta * Integrity + (1- \alpha - \beta) * Logicality
\end{equation}

\subsection{Story Aggregation}
% Describe the fact clustering algorithm, especially the distance measure and features that we used to calculate the distance. Describe the fact aggregation rule (the big table). Discuss the potential issues such as the perception cost. 

For now, the story pieces in our generated data story only convey single fact.
However, the compound fact is the common used fact that consists of multiple primitive facts \cite{amar2005low, chen2009toward}.
To keep the story concise, we aggregate the story by merging single facts into a compound one.
The story aggregation process consists of three major steps: (1)similarity measuring, (2)hierarchical clustering, and (3) fact merging.

First, we measures the similarity between data facts using the overlap similarity for categorical data \cite{boriah2008similarity}.
The overlap similarity of the \textit{type} is 0 when types of two facts are no match, and 1 when the attribute values match.
For the \textit{measure} and the \textit{group-by}, the similarity is the proportion of the fields in common.
For the \textit{subspace} and the \textit{focus}, we use the the fraction of union covered by intersection for similarity calculation.
The similarity in total is the sum of these five results.

Then, we aggregate the data facts into a hierarchical structure based on the similarity using hierarchical clustering technique.
After clustering, the pairs of leaf nodes, such as the dashed box in fig, are the potential facts to be merged.
These pairs of facts are ranked according to the similarity. 
The more similar facts have more tendency to be merged.
Calliope provides a slider bar that allows users to control the level of story aggregation in percentage, with a value of 0\% to present single facts, and a value of 100\% to merge all pairs of data facts.

To present the compound fact, Calliope merge facts in two aspects, including visualization and natural language.
For simplicity, we define a rule table for each combinations of two fact types.
In the table, we choose chart type for compound fact according to the intersection of chart candidates for each primitive fact type.
We also merge the fact tuples that have no conflict between each other.
If there is no common chart type between two facts or conflict in the fact tuples, we simply place the two visualization by juxtaposition.
For example, there is a trend fact and a extreme fact share same \textit{measure}, \textit{subspace}, and \textit{group-by} shown in Fig.\ref{fig:aggregation}.
The difference is that the extreme fact has an additional \textit{focus} which highlight the maximum value.
Based on our rule table, both of these two facts can use the line chart to present the information.
As a result, the compound fact use line chart  which is shown in Fig.\ref{fig:aggregation}.
For the description of compound fact, we choose to join together two sentences from both primitive facts.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/aggregation.png}
    \caption{Compound fact} 
    \label{fig:aggregation}
\end{figure}

Up to this point, Calliope does not consider the perception cost during the fact merging \cite{hullman2013deeper}.
Besides, the natural language in the compound fact may has redundancy, which can be solved by NLP techniques such as coreference resolution \cite{ng2002improving}.
We leave these questions in the future work.

==> sections-back/4-engine.tex <==
\section{Story Generation Engine}
\label{sec:engine}

In this section, we describe the technique details of the data story generation engine in Calliope system. We first introduce the definitions of different types of data facts and their importance measures followed by the details of the proposed story generation algorithm.

\subsection{Data Facts}
% (Describe the definition of each data fact.  Describe how did we calculate the significance and information of a fact. )

Based on our preliminary study and formative work \cite{wang2019datashot}, Calliope provides a formal model for representing data facts.
In definition, a data fact consist of a five-tuple, including \textit{type}, \textit{measure}, \textit{subspace}, \textit{group-by} and \textit{focus}.
$$
fact := (type, measure, subspace, groupby, focus)
$$

The \textit{type} definition identifies the fact type from 10 pre-defined taxonomies, including value, difference, proportion, trend, categorization, distribution, rank, association, extreme and outlier.
These 10 types derive from our preliminary survey on data videos and several formative works \cite{wang2019datashot, chen2009toward}. 
The \textit{measure} determines which numerical field and aggregation function to use as the measurement in the fact.
The \textit{subspace} specifies the range of data that fulfill a filter condition.
The \textit{group-by} groups records that have same value in categorical or temporal fields into summary records.
The \textit{focus} highlights the specific information in the subspace.

Table \ref{tab:fact_table} summarizes the rules to construct the data fact for each fact type.
As shown in the table, \textit{measure}, \textit{group-by} and \textit{focus} are not necessary for all fact types.
The definition of each fact type are depicted in the following list.
To explain the meaning of each fact type, we use a sample spreadsheet about automatic sales.
The columns' information is shown in Table \ref{table:tabledetail}.

\begin{table}[htb]
    \label{table:tabledetail}
    \caption{The information of columns in the sample}
    \centering
    \small
    \begin{tabular}{ccl}
    \hline
    field name & type & description \\ \hline
    Sales & numerical & automobile sales \\ 
    Income & numerical & automobile income \\ 
    Category & categorical & types of automobile (e.g. SUV, Compact) \\ 
    Brand & categorical & brands of automobile (e.g. BMW, Ford) \\ 
    Year & temporal & year of Sales (2007-2011) \\ \hline
    \end{tabular}
\end{table}

\begin{itemize}

    \item \textbf{Value} is defined on (\textit{measure}, \textit{subspace}).
    It derives the value according to the \textit{measure} in \textit{subspace}. 
    E.g. Show total sales in Brand Ford.
    
    \item \textbf{Difference} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It compares the \textit{measure} of two \textit{focus} on \textit{group-by} in \textit{subspace}.
    E.g. Compare difference between sales of SUV and Compact in Brand BMW.
    
    \item \textbf{Proportion} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It shows the proportion of the \textit{measure} in the \textit{focus} from all \textit{group-by}s in \textit{subspace}.
    E.g. Show proportion of SUV in total sales of Brand Ford.
    
    \item \textbf{Trend} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}).
    It shows the \textit{measure} order by the temporal \textit{group-by} in \textit{subspace}.
    E.g. Show the trend of sales in Brand Ford order by year.
    
    \item \textbf{Categorization} is defined on (\textit{subspace}, \textit{group-by}).
    It lists all \textit{group-by}s in \textit{subspace}.
    E.g. Show all categories contained in Brand Ford.
    
    \item \textbf{Distribution} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}).
    It shows the \textit{measure} of each \textit{group-by} in \textit{subspace}. 
    E.g. Show the sales of each category in Brand Ford.
    
    \item \textbf{Rank} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It lists all \textit{group-by} order by \textit{measure} in \textit{subspace} and \textit{focus} on the top rank.
    E.g. List the sales rank of brand in 2011.
    
    \item \textbf{Association} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}).
    It shows the relation between two \textit{measure}s by \textit{group-by} in \textit{subspace}.
    E.g. Show the relationship between sales and income in each brand in 2011.
    
    \item \textbf{Extreme} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It shows the \textit{measure} of each \textit{group-by} in \textit{subspace} and \textit{focus} on the extreme.
    E.g. Show the best-selling category in Brand Ford.
    
    \item \textbf{Outlier} is defined on (\textit{measure}, \textit{subspace}, \textit{group-by}, \textit{focus}).
    It shows the \textit{measure} of each \textit{group-by} in \textit{subspace} and \textit{focus} on the outlier.
    E.g. Show the outlier of sales by year in Brand Ford.
    
\end{itemize}

According to this fact definition, We describe a single data fact using a JSON specification in Calliope.
Based on the automobile spreadsheet, we demonstrate a \textit{Proportion} fact in Listing \ref{lst:json}.
The \textit{measure} of the fact is total sum of ``Sales".
The \textit{subspace} is the records when ``Brand" is equal to ``Ford".
The \textit{group-by} divide the subspace by ``Category", and the \textit{focus} is the records when when ``Category" is equal to ``SUV".
The meaning of this specification is to show the proportion fact about total Sales of SUV in the Brand Ford.

\begin{lstlisting}[caption=JSON specification of a data fact,
basicstyle=\small, label={lst:json}, language=json,firstnumber=1]
{
    "type": "proportion",
    "measure": [{"field": "Sales", "aggregate": "sum"}],
    "subspace": [{"field": "Brand", "value": "Ford"}],
    "group-by": [{"field": "Category"}],
    "focus": [{"field": "Category", "value": "SUV"}]
}
\end{lstlisting}

In addition the basic fact defination, data facts also have \textit{parameter} to explain the status of the fact, such as increasing or decreasing in the \textit{trend} fact.
Table \ref{tab:fact_table} displays all \textit{parameter} in 10 fact types.
These \textit{parameter}s can be derived from the data and fact specification directly.
With the \textit{parameter}, we can generate natural language for each fact. 
The detail of facts to natural language will be descripted in Section 5.2.1.

\begin{table*}[t]
    \caption{Data Facts}
    \label{tab:fact_table}
    \small
    \def\arraystretch{1.2}
    \begin{tabular}{|l|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|l|p{7.7cm}|}
    \hline
    fact type & \multicolumn{1}{l|}{measure} & \multicolumn{1}{l|}{subspace} & \multicolumn{1}{l|}{group-by} & \multicolumn{1}{l|}{ focus } & parameter & sentence template \\ \hline
    Value & O & O & X & X & derived value & The \{\{aggregate\}\} \{\{measure\}\} is \{\{parameter\}\} when \{\{subspace\}\}. \\ \hline
    Difference & O & O & O & O & difference value & \begin{tabular}[c]{@{}l@{}}The difference between \{\{focus{[}1{]}\}\} and \{\{focus{[}2{]}\}\} regarding to their \\ \{\{aggregate\}\} \{\{measure\}\} is \{\{parameter\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Proportion & O & O & O & O & percentage & \begin{tabular}[c]{@{}l@{}}The \{\{focus\}\} accounts for \{\{parameter\}\} of the \{\{aggregate\}\} \\ \{\{measure\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Trend & O & O & O & X & increasing/decreasing & \begin{tabular}[c]{@{}l@{}}The trend of \{\{aggregate\}\} \{\{measure\}\} over \{\{group-by\}\} is \\ \{\{parameter\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Categorization & X & O & O & X & number of categories & \begin{tabular}[c]{@{}l@{}}Given \{\{subspace\}\}, there are \{\{parameter\}\} \{\{group-by\}\}(s) \\ which are \{\{C\_1\}\}, \{\{C\_2\}\}, \{\{...\}\}, and \{\{C\_n\}\}.\end{tabular} \\ \hline
    Distribution & O & O & O & X & N/A & \begin{tabular}[c]{@{}l@{}}The distribution of the \{\{aggregate\}\} \{\{measure\}\} over different \\ \{\{group-by\}\}(s) shows an overview of the data when \{\{subspace\}\}.\end{tabular} \\ \hline
    Rank & O & O & O & O & N/A & \begin{tabular}[c]{@{}l@{}}In the \{\{aggregate\}\} \{\{measure\}\} ranking of different \{\{group-by\}\}(s), \\ the top three \{\{group-by\}\}(s) are \{\{focus{[}0{]}\}\}, \{\{focus{[}1{]}\}, \{\{focus{[}2{]}\}\},\\ when \{\{subspace\}\}.\end{tabular} \\ \hline
    Association & O & O & O & X & correlation value & \begin{tabular}[c]{@{}l@{}}The Pearson correlation between the \{\{measure{[}1{]}\}\} and the \\ \{\{measure{[}2{]}\}\} is \{\{parameter\}\} in case of \{\{subspace\}\}.\end{tabular} \\ \hline
    Extreme & O & O & O & O & \begin{tabular}[c]{@{}l@{}}0: max/min\\ 1: extreme value\end{tabular} & \begin{tabular}[c]{@{}l@{}}Given \{\{subspace\}\}, the \{\{parameter{[}0{]}\}\} value of the \{\{aggregate\}\} \\ \{\{measure\}\}is \{\{parameter{[}1{]}\}\} when \{\{group-by\}\} is \{\{focus\}\}.\end{tabular} \\ \hline
    Outlier & O & O & O & O & outlier value & \begin{tabular}[c]{@{}l@{}}The\{\{aggregate\}\} \{\{measure\}\} of \{\{focus\}\} is an outlier when compare \\ with that of other \{\{group-by\}\}(s) when \{\{subspace\}\}.\end{tabular} \\ \hline
    \end{tabular}
\end{table*}

Calliope calculate the importance score $I(f)$ for a data fact $f$ to measure the value of fact.
The score contains two aspects: information importance ${\rm Info}(f)$ and significance importance ${\rm Sig}(f)$.
The importance score for each fact is:

\begin{equation}
    I(f) = {\rm Sig}(f) \cdot {\rm Info}(f)
\end{equation}

\textbf{Information importance} ${\rm Info}(f)$ is measured by Shannon entropy \cite{shannonentropy}, which is also called the self-information of a data fact.
The information importance should be high when an unlikely data fact is observed in spreadsheet.
It is calculated as follows, where $X$ is the scope of the data:

\begin{equation}
{\rm Info}(f) = -log_2(P(X))
\end{equation}

According our fact definition, the \textit{subspace} and the \textit{focus} are the only two elements that related to the scope of the data $X$.
So the probability of $X$ is then determined by the product of the probability of \textit{subspace} and conditional probability of \textit{focus} given \textit{subspace}:

\begin{equation}
P(X) = P(subspace) \cdot P(focus | subspace)
\end{equation}

For now, we only support at most 2 fields in the subspace of the fact.
The following formulation is to calculate the probability of the subspace:

% \begin{equation}
% P(subspace)  =  P(field = K)
% \end{equation}
\begin{equation}
P(subspace)=\frac{1}{\sum_{i=0}^{2} C(n, i)}\cdot\prod_{i=1}^{k}\frac{count({subspace}_i)}{count(all)}
\end{equation}
The former item is the probability of the occurence of the \textit{subspace}, where $n$ is the count of categorical and temporal fields in the spreadsheet, and $C(n,i)$ is the number of $i$-combinations from $n$ fields. 
The latter item is the probability of the \textit{subspace}, where $count({subspace}_i)$ is the count of records which fulfills the $i$th condition in \textit{subspace} and $count(all)$ is the total count of the spreadsheet.
When the \textit{subspace} includes two fields, we assume they are independent to each other.
So we calculate the product of the probabilities of two \textit{subspace}s.

The conditional probability of \textit{focus} given \textit{subspace} is determined by the fraction of the count of \textit{subspace} covered by the count of \textit{focus}:

\begin{equation}
P(focus|subspace)= \frac{count(focus)}{count(subspace)}
\end{equation}

\textbf{Significance importance} ${\rm Sig}(f)$ is the measurement from the statistical aspect. 
To determine the importance of fact, significance is the weight for the information importance in [0, 1].
For instance, if a trend fact is steady with no obvious increasing or decreasing, it should have a low significance close to 0.
In contrast, a fact shows a clear rising trend line should get a high significance close to 1.
We calculate the significance importance of the fact using the methods in formative works \cite{ding2019quickinsights, tang2017extracting, wang2019datashot}.

\subsection{Story Generation Algorithm}
% First describe the algorithm overview via pseudocode and explain the algorithm pipeline by important steps.

We introduce Monte Carlo Tree Search

There are 4 steps in each search iteration: (1) Selection, (2) Expansion, (3) Simulation, (4) Backpropagation.
These steps are grouped into two policies, including logic tree policy and default policy.
The total generation algorithm is summarized in pseudocode in Algorithm \ref{alg:generation}.

\begin{algorithm}[htb]
    \label{alg:generation}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{Data from spreadsheet}
    \Output{Story with a sequence of data facts}
    % \KwResult{Write here the result }
    $f_0$ $\leftarrow$ InitalFact($data$)\;
    $story$ $\leftarrow$ [$f_0$]\;
    \While{length(story) < max}{
        \While{within computational time}{
            ($f_l$,$r_l$) $\leftarrow$ LogicTreePolicy($story$)\;
            $\Delta$ $\leftarrow$ DefaultPolicy($story(f_l, r_l)$)\;
            Backup(($f_l$,$r_l$), $\Delta$)\;
        }
        $story$.insert(BestChild($story$))\;
    }
    $story$ $\leftarrow$ Aggregation($story$)\;
    \Return $story$\;
    \caption{Data Story Generation}
\end{algorithm}
$f_0$ is the first fact and the root node corresponding to the $story$.
$f_l$ and $r_l$ is the last fact and relation reached during the logic tree policy, which will be introduced in Section 4.2.1.
$\Delta$ is the reward for terminal $story$ by running the default policy.
The result of the overall search BestChild($story$) is the fact and relation that leads to the best reward.
So we take the result to append the current $story$.
After all iterations are finished, we get the final generated $story$ and aggregate it using the method mentioned in Section 4.3.

\subsubsection{Logic Calculation}
% Describing how did we ensures the story logic and reduce the search space. Describe the statistics that we summarized based on the preliminary survey.

According to preliminary data videos survey and formative corpus study \cite{wolf2005representing}, we summarize 6 discourse relations in data stories.
We list them in Table \ref{table:relation}.

\begin{table}[]
    \centering
    \label{table:relation}
    \caption{6 discourse relations and their example templates in data stories.}
    \begin{tabular}{ll}
    \hline
    relation & example template \\ \hline
    similarity & \{\{$Fact_a$\}\}. \{\{$Fact_b$\}\}. \\ 
    temporal & \{\{$Fact_a$\}\}. After that, \{\{$Fact_b$\}\}. \\ 
    contrast & \{\{$Fact_a$\}\}. However, \{\{$Fact_b$\}\}. \\ 
    cause-effect & \{\{$Fact_a$\}\}. The reason is \{\{$Fact_b$\}\}. \\ 
    elaboration & \{\{$Fact_a$\}\}. Furthermore, \{\{$Fact_b$\}\}. \\ 
    generalization & \{\{$Fact_a$\}\}. In general, \{\{$Fact_b$\}\}. \\ \hline
    \end{tabular}
\end{table}

Initial fact:

\subsubsection{Reward Function}
Describing the reward function followed by the details of each terms in the function. The key is to clearly describe the design rationale of each term.

We define the information entropy of the data story as $H(story)$.

\begin{equation}
H(story) = E(I(F)) = \sum_{i=1}^{n} { P(f_i) \cdot I(f_i) }
\end{equation}
$I(f_i)$ is the quantity of information for the $i$th fact and the $X$ is the data of the fact.

Based on the information entropy, we add significance into the formulation to calculate the importance score of the story $I(S)$.

\begin{equation}
I(S)  = E(S(F) \cdot I(F)) =  \sum_{i=1}^{n} { P(f_i) \cdot S(f_i) \cdot I(f_i) }
\end{equation}

The coefficient of user preference $w_{S}$ includes three parameters: logicality, diversity and integrity.

\textbf{Logicality}

\begin{equation}
Logicality = \frac{1}{n}\sum_{i=1}^{n-1}P\left(r_{i-1} | f_{i}\right)
\end{equation}

\textbf{Diversity}

\begin{equation}
Diversity = \frac{count(type)}{\max (length(S),10)} *-\frac{\sum_{j=1}^{i} \hat{p}_{j} \cdot \ln \left(\hat{p}_{j}\right)}{\ln (s)} 
\end{equation}

\textbf{Integrity}

\begin{equation}
Integrity = \frac{count_{cell}(\bigcup\limits_{i=0}^{n-1} f_{i})}{count_{cell}(data)}
\end{equation}

The total story reward is the importance score of the story with the coefficient of user preference.
Bringing each parameters together, the final $reward$ is:

\begin{equation}
reward =  (\alpha \cdot Diversity  + \beta \cdot Integrity + \gamma \cdot Logicality) \cdot I(S)
\end{equation}
where $\alpha$, $\beta$ and $\gamma$ is the weight in [0,1] and the sum of them is equal to 1.
Users can determine the value by interaction in the storyline view.
The interaction detail will be introduced in Section 5.1.

\subsection{Story Aggregation}
% Describe the fact clustering algorithm, especially the distance measure and features that we used to calculate the distance. Describe the fact aggregation rule (the big table). Discuss the potential issues such as the perception cost. 

For now, the story pieces in our generated data story only convey single fact.
However, the compound fact is the common used fact that consists of multiple primitive facts \cite{amar2005low, chen2009toward}.
For instance, "The trend of sales is decreasing and the maximum of sales is in 2007" is a compound fact that involves a trend fact and an extreme fact.
To keep the story concise, Calliope provides an option for users to aggregate the story by merging single facts into a compound one automatically.

The story aggregation process consists of three major steps: (1) similarity measuring, (2) hierarchical clustering, and (3) fact merging.

First, we measures the similarity between data facts using the overlap similarity for categorical data \cite{boriah2008similarity}.
The overlap similarity of the \textit{type} is 0 when types of two facts are no match, and 1 when the attribute values match.
For the \textit{measure} and the \textit{group-by}, the similarity is the proportion of the fields in common.
For the \textit{subspace} and the \textit{focus}, we use the the fraction of union covered by intersection for similarity calculation.
The similarity in total is the sum of these five results.

Then, we aggregate the data facts into a hierarchical structure based on the similarity using hierarchical clustering technique.
After clustering, the pairs of leaf nodes, such as the dashed box in fig, are the potential facts to be merged.
These pairs of facts are ranked according to the similarity. 
The more similar facts have more tendency to be merged.
Calliope provides a slider bar that allows users to control the level of story aggregation in percentage, with a value of 0\% to present single facts, and a value of 100\% to merge all pairs of data facts.

To present the compound fact, Calliope merge facts in two aspects, including visualization and natural language.
For simplicity, we define a rule table for each combinations of two fact types.
In the table, we choose chart type for compound fact according to the intersection of chart candidates for each primitive fact type.
We also merge the fact tuples that have no conflict between each other.
If there is no common chart type between two facts or conflict in the fact tuples, we simply place the two visualization by juxtaposition.
For example, there is a trend fact and a extreme fact share same \textit{measure}, \textit{subspace}, and \textit{group-by} shown in Fig.\ref{fig:aggregation}.
The difference is that the extreme fact has an additional \textit{focus} which highlight the maximum value.
Based on our rule table, both of these two facts can use the line chart to present the information.
As a result, the compound fact use line chart  which is shown in Fig.\ref{fig:aggregation}.
For the description of compound fact, we choose to join together two sentences from both primitive facts.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/aggregation.png}
    \caption{Compound fact} 
    \label{fig:aggregation}
\end{figure}

Up to this point, Calliope does not consider the perception cost during the fact merging \cite{hullman2013deeper}.
Besides, the natural language in the compound fact may has redundancy, which can be solved by NLP techniques such as coreference resolution \cite{ng2002improving}.
We leave these questions in the future work.

==> sections-back/5-editor.tex <==

\subsection{Storyline View}
% Describe the design details of the storyline view.
The storyline view(Fig.~\ref{fig:ui}-1) contains two panels, the story configuration panel(Fig.~\ref{fig:ui}-1(a)) and the story pieces panel(Fig.~\ref{fig:ui}-1(b)). The story configuration panel is where users upload data, tweak parameters for the generated story, such as the story length, the chart diversity and the tolerable time limitation of the generation. The chart diversity represents chart type diversities of each fact type in the generated story ranging from zero to one. Particularly, the value of zero means that each type of facts maps to only one chart type in the generated result. When users increase the value with the slider, more chart types will show up for each fact type in the story. 

In the reward view within the story configuration panel, users can also set up their preference for the reward of the story generation algorithm, including three key parameters: logicality, diversity and integrity. A chart is implemented with one movable circle and three fixed circles to encode the relation among the generated story and the three key parameters.
Here, the circle $S$ represents the story, and three fixed circles representing three parameters shape a circular area, and the distances between $S$ and three parameter circles capture the weights of each parameter. While moving the circle $S$, the parameter circles that are closer to $S$ will obtain higher weights and more attention when generating.

After clicking the ``Generate Story" button in the configuration panel, \name will yield a sequence of data facts in a logic order and line them in the story pieces panel successively. 
Each piece in this panel shows a fact of data with visualization and description. 
For easy revision, \name allows users to add, remove or re-arrange these fact pieces by simple interaction, as well as edit the statement of facts. When a specific fact piece is selected, its details will show up in the fact view, where users can modify it to meet their needs. These actions will apply in all the other views accordingly to reduce repetitive modification. 

\subsection{Fact View}
% Describe the representation methods of the facts in detail.
The fact view (Fig.~\ref{fig:ui}-2) is a detailed view that not only represent the selected story piece but also enables users to customize this fact by changing the configuration. 
Fact's configuration items include the following: \textit{fact type}, \textit{visualization}, \textit{measure},\textit{subspace}, \textit{breakdown}, and \textit{focus}. Different fact types may have specific combination of the configuration items mentioned above according to table~\ref{tab:fact}.
Through the adjustment of these configuration items, the nature language(\ref{5.2.1}) and the visualization(\ref{5.2.2}) of the fact will be generated in real time. Also, the information quantity and significance score of the selected fact will be updated accordingly. 

\subsubsection{Facts to Nature Language}
Each facts is equivalent to a context free grammar which can be used to generate nature language. Describe how the description text are generated for each fact type.
\label{5.2.1}

\subsubsection{Facts to Visualization}
% Describe how to properly visualize a fact based on our preliminary survey. Not only mention our statistic results but also describe our alternative designs used for ensuring the visual diversity.

% chart diversity
Based on our preliminary survey, we design a rule based method to match fact types with different chart types. For ensuring the visual diversity, we add some alternative designs of each basic chart based on statistical results. For example, donut chart and half donut chart can be  the variants of the basic pie chart for users to choose.

% chart mapping
The visualization changes accordingly with the adjustment of fact configuration. Among the configuration items, \textit{subspace} subspace is used to specify the range of data to be visualized, \textit{measure} and \textit{groupby} respectively correspond to the measure and dimension that make up the chart, and \textit{focus} is used as the highlighted part in the chart.
\label{5.2.2}

\subsection{Story Visualization View}
The story visualization view provides a variety of visualization forms to represent the generated data story line for different application scenarios. In particular, a summarization view is first provided to give a textual briefing of the story to help users obtain data insights at a glance. It shows the data coverage rate, total number of data facts in the story, and a textual description of the story. 

To facilitate an efficient story exploration on tablets and smart phones, a storyline view and a mobile view are respectively developed. The visualizations and textual descriptions of the facts in the story are grouped together and horizontally aligned in a row in the storyline view and are showed one at a time in the mobile view. Users can swipe on the touch screen to scroll the horizontal storyline in the storyline view or switch to another fact in the mobile view to navigate through the story. 

Finally, a fact-sheet view is also introduced, in which the visual and textual representation of all the facts are organized into a poster that can be directly downloaded and printed. This view supports an easy offline usage of the generation results. A layout algorithm is designed to enable an efficient and aesthetic representation of the story facts. Formally, the algorithm is designed to optimize the following objective: 

\begin{equation}
    f = f_s + f_d
    \label{eq:optimize}
\end{equation}
where $f_s$ indicates how the areas of each fact take up in the fact sheet in proportion of their importance scores, shown in Eq.(\ref{eq:opti_area}); $f_d$ measures whether the layout of the fact sheet matches the guideline of low intra-row distances and high inter-row distances defined in Eq.(\ref{eq:opti_layout}).
\begin{equation}
    f_s = \frac{\sum_{i=1}^{n} s_i \times a_i }{\sum_{i=1}^{n} a_i }
    \label{eq:opti_area}
\end{equation}
where $n$ is the number of facts in the generated story; $s_i$ is the importance score of $i$-th fact derived from the story generation algorithm, and $a_i$ is the area $i$-th fact occupied. With $f_s$, we expect that facts with higher scores would involve larger areas to attract enough attention from readers for they bring more information.

Here we denote the layout of fact sheet with $n$ facts as $C = \{C_1, C_2, \cdots, C_k\}$, where $k$ is the number of rows in the fact sheet. Formally, $f_d$ is calculated as follows:
\begin{equation}
f_d = f_d^{inter} - f_d^{intra}
\label{eq:opti_layout}
\end{equation}
\begin{equation}
f_d^{inter} = \frac{\sum_{1 \leq j < |C|} d(C_j, C_j+1)}{|C|-1}
\label{eq:opti_inter}
\end{equation}
\begin{equation}
f_d^{intra} = \frac{\sum_{C_j \in C} \sum_{1 \leq i < |C_i|} d(x_i, x_{i+1})} {n - |C|}
\label{eq:opti_intra}
\end{equation}
where $d$ measures the distance between two facts. To obtain it, we first calculate the similarity between two facts as described in Sec.~\ref{4.3} and then minus it from one, indicating low similarities lead to high distances. As for the distance between two rows, we identify it as the distance between two adjacent facts connecting rows. Finally, $f_d$ is derived by subtracting $f_d^{intra}$, the average distance inside rows, from $f_d^{inter}$, the average distance between rows. With higher value, $f_d$ represents a more compact layout of a fact sheet in terms of the logic relations among facts through the generated story.
\label{StoryView}


\subsection{Interactions}
% Describe the interactions of the system.

\name provides a set of interaction methods to support the data story generation, fact exploration, story visualization and publishing to the public web.

{\bf Data story generation.} \name allows users to fine-tune several details of the story in the story configuration panel within the storyline view. For the length of the story generated by \name, the chart diversity for each fact type and the time limitation of generation, users can drag the sliders of each parameter to pick a specific value from the given range. As for the reward preference for the generation, user can drag the circle $S$ which presents the story in the reward panel, to a position where distances between the story circle and three parameter nodes capture the relevant weights accordingly. After all parameters settled, users can click the ``Generate Story" button and wait for the story from \name in a few seconds. With the generated story, \name allows users to add a new fact piece or remove current fact pieces by clicking buttons, or re-order the fact pieces by simple drag-and-drop interaction in the story pieces panel. Editing the fact description is also enabled in the story pieces panel. All actions will apply in all the other views accordingly to reduce repetitive modification. 

{\bf Modifying data fact.} The fact view enables users to customize the Currently selected fact by changing the fact's configuration. 
Fact view provides selectors for \textit{fact type}, \textit{visualization}, \textit{measure},\textit{subspace}, \textit{breakdown}, and \textit{focus}. When adjusting these configuration items, visual and textual representations of the current fact will be modified. 

{\bf Choosing visualization form and publishing.} 
\name allows user to switch between all the visualization forms mentioned in~\ref{StoryView} in the story visualization view.
By clicking the ``share" button, \name can automatically generate an online access link and a code snippet that can be embedded in other web pages for the generated data story represented in its current visualization form. When the user clicks the copy button, the online link or the code snippet will be copied accordingly. If others visit the link, they can access this data story. As for the generated 
code snippet, user can easily embed this data story into his own web page by inserting the snippet into it.

\label{5.4}

==> sections-back/5-story.tex <==
\section{Data Story Editor}
\label{sec:editor}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/UI.png}
  \caption{The story editor of \name system contests of three major views: (1) the storyline view for story configuration, generation and storyline editing, (2) the fact view for fact editing, and (3) the story visualization view for the visual data story preview and sharing.} \label{fig:ui}
\end{figure}

In this section, we describe the design details of each views in the data story editor and the corresponding interactions of the system. 

\subsection{User Interface}
The story editor, as shown in Fig.~\ref{fig:ui}, consists of three major views: the storyline view (Fig.~\ref{fig:ui}-1), the fact view (Fig.~\ref{fig:ui}-2), and the story visualization view (Fig.~\ref{fig:ui}-3). In the storyline view, a user can upload a spreadsheet, set the story generation goal, and adjust the reward function in a group of configuration panels (Fig.~\ref{fig:ui}-1(a)). The generated data facts are shown in a row (Fig.~\ref{fig:ui}-1(b)), in which a user can remove a fact or change the generated narrative order based on his/her own preferences. Each fact is visualized by a chart and captioned by a generated text description (\textbf{R3}). When a fact is selected, its data details, importance measures, and visual and textual representations will be shown in the fact view, which are also editable (\textbf{R4}). The generated data story can be visualized in the story visualization view through three visualization modes: (1) the storyline mode, (2) the swiper mode, and (3) the fact sheet mode, respectively designed for representing the story on laptops/tablets, smart phones, and in printouts to facilitate a flexible story communication and sharing (\textbf{R5}).

Let's consider the following scenario for using \name system. Jean is a data journalist. Her primary job is to tracing important news events, collect, analyze, and visualize the corresponding data to write news stories with the data support. Her job frequently requires a quick response to emergencies, but data analysis and visualization usually take days to finish. She uses \name to help her on these tasks. Recently, she is monitoring the public health emergency on the propagation of CoVID-19 virus in China. A data containing everyday infections and deaths in different provinces and cities are collected. She uploads the data into \name system, sets the story length as 6 (i.e., contains at most 6 data facts) in the story configuration panel, and clicks the generate button. Only after a few seconds, the system automatically outputs a sequence of related data facts represented by charts and captioned by text in a logic order in the storyline view. She clicks a generated fact to edit it in the fact view, where she can change the generated description, chart and the fact types, and the data details based on her own observations and preferences. After a few edits on the story facts, Jean switched the visual representation style to the swiper mode in the story visualization view and shared the results with her colleague via a link by clicking the share button for a future discussion.

% \subsection{Storyline View}
% % Describe the design details of the storyline view.
% The storyline view(Fig.~\ref{fig:ui}-1) contains two panels, the story configuration panel(Fig.~\ref{fig:ui}-1(a)) and the story pieces panel(Fig.~\ref{fig:ui}-1(b)). The story configuration panel is where users upload data, tweak parameters for the generated story, such as the story length, the chart diversity and the tolerable time limitation of the generation. The chart diversity represents chart type diversities of each fact type in the generated story ranging from zero to one. Particularly, the value of zero means that each type of facts maps to only one chart type in the generated result. When users increase the value with the slider, more chart types will show up for each fact type in the story. 

% In the reward view within the story configuration panel, users can also set up their preference for the reward of the story generation algorithm, including three key parameters: logicality, diversity and integrity. A chart is implemented with one movable circle and three fixed circles to encode the relation among the generated story and the three key parameters.
% Here, the circle $S$ represents the story, and three fixed circles representing three parameters shape a circular area, and the distances between $S$ and three parameter circles capture the weights of each parameter. While moving the circle $S$, the parameter circles that are closer to $S$ will obtain higher weights and more attention when generating.

% After clicking the ``Generate Story" button in the configuration panel, \name will yield a sequence of data facts in a logic order and line them in the story pieces panel successively. 
% Each piece in this panel shows a fact of data with visualization and description. 
% For easy revision, \name allows users to add, remove or re-arrange these fact pieces by simple interaction, as well as edit the statement of facts. When a specific fact piece is selected, its details will show up in the fact view, where users can modify it to meet their needs. These actions will apply in all the other views accordingly to reduce repetitive modification. 

\subsection{Fact View}
% Describe the representation methods of the facts in detail.
The fact view (Fig.~\ref{fig:ui}-2) is a detailed view that not only represent the selected story piece but also enables users to customize this fact by changing the configuration. 
Fact's configuration items include the following: \textit{fact type}, \textit{visualization}, \textit{measure},\textit{subspace}, \textit{breakdown}, and \textit{focus}. Different fact types may have specific combination of the configuration items mentioned above according to table~\ref{tab:fact}.
Through the adjustment of these configuration items, the nature language(\ref{5.2.1}) and the visualization(\ref{5.2.2}) of the fact will be generated in real time. Also, the information quantity and significance score of the selected fact will be updated accordingly. 

\subsubsection{Facts to Nature Language}
Each facts is equivalent to a context free grammar which can be used to generate nature language. Describe how the description text are generated for each fact type.
\label{5.2.1}

\subsubsection{Facts to Visualization}
% Describe how to properly visualize a fact based on our preliminary survey. Not only mention our statistic results but also describe our alternative designs used for ensuring the visual diversity.

% chart diversity
Based on our preliminary survey, we design a rule based method to match fact types with different chart types. For ensuring the visual diversity, we add some alternative designs of each basic chart based on statistical results. For example, donut chart and half donut chart can be  the variants of the basic pie chart for users to choose.

% chart mapping
The visualization changes accordingly with the adjustment of fact configuration. Among the configuration items, \textit{subspace} subspace is used to specify the range of data to be visualized, \textit{measure} and \textit{groupby} respectively correspond to the measure and dimension that make up the chart, and \textit{focus} is used as the highlighted part in the chart.
\label{5.2.2}

\subsection{Story Visualization View}
The story visualization view provides a variety of visualization forms to represent the generated data story line for different application scenarios. In particular, a summarization view is first provided to give a textual briefing of the story to help users obtain data insights at a glance. It shows the data coverage rate, total number of data facts in the story, and a textual description of the story. 

To facilitate an efficient story exploration on tablets and smart phones, a storyline view and a mobile view are respectively developed. The visualizations and textual descriptions of the facts in the story are grouped together and horizontally aligned in a row in the storyline view and are showed one at a time in the mobile view. Users can swipe on the touch screen to scroll the horizontal storyline in the storyline view or switch to another fact in the mobile view to navigate through the story. 

Finally, a fact-sheet view is also introduced, in which the visual and textual representation of all the facts are organized into a poster that can be directly downloaded and printed. This view supports an easy offline usage of the generation results. A layout algorithm is designed to enable an efficient and aesthetic representation of the story facts. Formally, the algorithm is designed to optimize the following objective: 

\begin{equation}
    f = f_s + f_d
    \label{eq:optimize}
\end{equation}
where $f_s$ indicates how the areas of each fact take up in the fact sheet in proportion of their importance scores, shown in Eq.(\ref{eq:opti_area}); $f_d$ measures whether the layout of the fact sheet matches the guideline of low intra-row distances and high inter-row distances defined in Eq.(\ref{eq:opti_layout}).
\begin{equation}
    f_s = \frac{\sum_{i=1}^{n} s_i \times a_i }{\sum_{i=1}^{n} a_i }
    \label{eq:opti_area}
\end{equation}
where $n$ is the number of facts in the generated story; $s_i$ is the importance score of $i$-th fact derived from the story generation algorithm, and $a_i$ is the area $i$-th fact occupied. With $f_s$, we expect that facts with higher scores would involve larger areas to attract enough attention from readers for they bring more information.

Here we denote the layout of fact sheet with $n$ facts as $C = \{C_1, C_2, \cdots, C_k\}$, where $k$ is the number of rows in the fact sheet. Formally, $f_d$ is calculated as follows:
\begin{equation}
f_d = f_d^{inter} - f_d^{intra}
\label{eq:opti_layout}
\end{equation}
\begin{equation}
f_d^{inter} = \frac{\sum_{1 \leq j < |C|} d(C_j, C_j+1)}{|C|-1}
\label{eq:opti_inter}
\end{equation}
\begin{equation}
f_d^{intra} = \frac{\sum_{C_j \in C} \sum_{1 \leq i < |C_i|} d(x_i, x_{i+1})} {n - |C|}
\label{eq:opti_intra}
\end{equation}
where $d$ measures the distance between two facts. To obtain it, we first calculate the similarity between two facts as described in Sec.~\ref{4.3} and then minus it from one, indicating low similarities lead to high distances. As for the distance between two rows, we identify it as the distance between two adjacent facts connecting rows. Finally, $f_d$ is derived by subtracting $f_d^{intra}$, the average distance inside rows, from $f_d^{inter}$, the average distance between rows. With higher value, $f_d$ represents a more compact layout of a fact sheet in terms of the logic relations among facts through the generated story.
\label{StoryView}


\subsection{Interactions}
% Describe the interactions of the system.

\name provides a set of interaction methods to support the data story generation, fact exploration, story visualization and publishing to the public web.

{\bf Data story generation.} \name allows users to fine-tune several details of the story in the story configuration panel within the storyline view. For the length of the story generated by \name, the chart diversity for each fact type and the time limitation of generation, users can drag the sliders of each parameter to pick a specific value from the given range. As for the reward preference for the generation, user can drag the circle $S$ which presents the story in the reward panel, to a position where distances between the story circle and three parameter nodes capture the relevant weights accordingly. After all parameters settled, users can click the ``Generate Story" button and wait for the story from \name in a few seconds. With the generated story, \name allows users to add a new fact piece or remove current fact pieces by clicking buttons, or re-order the fact pieces by simple drag-and-drop interaction in the story pieces panel. Editing the fact description is also enabled in the story pieces panel. All actions will apply in all the other views accordingly to reduce repetitive modification. 

{\bf Modifying data fact.} The fact view enables users to customize the Currently selected fact by changing the fact's configuration. 
Fact view provides selectors for \textit{fact type}, \textit{visualization}, \textit{measure},\textit{subspace}, \textit{breakdown}, and \textit{focus}. When adjusting these configuration items, visual and textual representations of the current fact will be modified. 

{\bf Choosing visualization form and publishing.} 
\name allows user to switch between all the visualization forms mentioned in~\ref{StoryView} in the story visualization view.
By clicking the ``share" button, \name can automatically generate an online access link and a code snippet that can be embedded in other web pages for the generated data story represented in its current visualization form. When the user clicks the copy button, the online link or the code snippet will be copied accordingly. If others visit the link, they can access this data story. As for the generated 
code snippet, user can easily embed this data story into his own web page by inserting the snippet into it.

\label{5.4}

% （3.20）*******************************************************

% \section{Data Story Generation and Visualization}
% In this section, we introduce the technique details of story generation algorithm and visualization methods. We start by describing a preliminary survey from which we learn some necessary priory knowledge that helps with the algorithm and visualization design. 

% \subsection{Data Story}
% Give a formal definition of data story in our context.

% \subsection{Data Story Generation}

% First give a formal definition about data story (i.e., a collection of facts). After that, describe the algorithm overview via pseudocode and explain the algorithm pipeline by important steps.

% \subsubsection{Logic Calculation}
% Describing how did we ensures the story logic and reduce the search space. Describe the statistics that we summarized based on the preliminary survey.

% \subsubsection{Reward Function}
% Describing the reward function followed by the details of each terms in the function. The key is to clearly describe the design rationale of each term.

% \subsubsection{Facts Aggregation}
% Describe the fact clustering algorithm, especially the distance measure and features that we used to calculate the distance. Describe the fact aggregation rule (the big table). Discuss the potential issues such as the perception cost. 


% \subsection{Storyline View}
% % Describe the design details of the storyline view.
% The storyline view(Fig.~\ref{fig:ui}-1) contains two panels, the story configuration panel(Fig.~\ref{fig:ui}-1(a)) and the story pieces panel(Fig.~\ref{fig:ui}-1(b)). The story configuration panel is where users upload data, tweak parameters for the generated story, such as the story length, the chart diversity and the tolerable time limitation of the generation. The chart diversity represents chart type diversities of each fact type in the generated story ranging from zero to one. Particularly, value of zero means that each type of facts maps to only one chart type in the generated result. When users increase the value with the slider, more chart types will show up for each fact type in the story. 

% In the reward view within the story configuration panel, users can also set up their preference for the reward of the story generation algorithm, including three key parameters: logicality, diversity and integrity. A chart is implemented with one movable circle and three fixed circles to encode the relation among the generated story and the three key parameters.
% Here, the circle $S$ represents the story, and three fixed circles representing three parameters shape a circular area, and the distances between $S$ and three parameter circles capture the weights of each parameter. While moving the circle $S$, the parameter circles that are closer to $S$ will obtain higher weights and more attention when generating.

% After clicking the ``Generate Story" button in the configuration panel, \name will yield a sequence of data facts in a logic order and line them in the story pieces panel successively. 
% Each piece in this panel shows a fact of data with visualization and description. For easy revision, \name allows users to add, remove or re-arrange these fact pieces by simple interaction, as well as edit the statement of facts. When a specific fact piece is selected, its details will show up in the fact view, where users can modify it to meet their needs. These actions will apply in all the other views accordingly to reduce repetitive modification. 


% \subsection{Fact View}
% % Describe the representation methods of the facts in detail.
% The fact view (Fig.~\ref{fig:ui}-2) is a detailed view that not only represent the selected story piece but also enable users to customize this fact by changing the configuration.
% The chart changes accordingly when the configuration item changes
% % The fact view(Fig.~\ref{fig:ui}-2) contains two panels, the fact configuration panel(Fig.~\ref{fig:ui}-2) and the story piece panel(Fig.~\ref{fig:ui}-2). 

% Fact's configuration items include the following: fact type, visualization, measure, subspace, groupby, focus.
% % 除了type和visualization，其他项跟着fact种类变化
% % 当fact type被更改时，所有的fact view中所有的配置内容会被清空，同时，每个fact对应的配置项的combination也会相应被更改
% And different fact types may have specific combination of the configuration items mentioned above according to table \ref{tab:fact_table}.
% Through the adjustment of these configuration items, the nature language(specific in 5.2.1) and the visualization(specific in 5.2.2) of the fact will be generated in real time. Also, the score of the fact will be updated accordingly. 

% \subsubsection{Facts to Nature Language}
% Each facts is equivalent to a context free grammar which can be used to generate nature language. Describe how the description text are generated for each fact type.

% \subsubsection{Facts to Visualization}
% % Describe how to properly visualize a fact based on our preliminary survey. Not only mention our statistic results but also describe our alternative designs used for ensuring the visual diversity.
% Based on our preliminary survey, we designed a rule based method to match fact types to different chart types. For ensuring the visual diversity, we have made some extensions to each basic chart based on statistical results. 
% For example, pie chart can be extended to donut chart, half donut chart, etc.
% % E.g. pie chart can be extended to donut chart, half donut chart, etc.
% The visualization changes accordingly when the configuration changes. Among the configuration items, ``subspace" is used to filter data, ``measure" is used as the measure in the chart, ``groupby" is used as the dimension in the chart, and ``focus" is used as the highlighted part in the chart.


% \subsection{Data Story Visualization}
% Callipoe system provides a variety of visualization forms to represent the generated data story line for different application scenarios. In particular, a summarization view is first provided to give a textual briefing of the story to help users obtain data insights at a glance. It shows the data coverage rate, total number of data facts in the story, and a textual description of the story. 

% To facilitate an efficient story exploration on tablets and smart phones, a storyline view and a mobile view are respectively developed. The visualizations and textual descriptions of the facts in the story are grouped together and horizontally aligned in a row in the storyline view and are showed one at a time in the mobile view. Users can swipe on the touch screen to scroll the horizontal storyline in the storyline view or switch to another fact in the mobile view to navigate through the story. 

% Finally, a fact-sheet view is also introduced, in which the visual and textual representation of all the facts are organized into a poster that can be directly downloaded and printed. This view supports an easy offline usage of the generation results. A layout algorithm is designed to enable an efficient and aesthetic representation of the story facts. Formally, the algorithm is designed to optimize the following objective: 

% \begin{equation}
%     f = f_s + f_d
%     \label{eq:optimize}
% \end{equation}
% where $f_s$ indicates how the areas of each fact take up in the fact sheet in proportion of their importance scores, shown in Eq.(\ref{eq:opti_area}); $f_d$ measures whether the layout of the fact sheet matches the guideline of low intra-row distances and high inter-row distances defined in Eq.(\ref{eq:opti_layout}).
% \begin{equation}
%     f_s = \frac{\sum_{i=1}^{n} s_i \times a_i }{\sum_{i=1}^{n} a_i }
%     \label{eq:opti_area}
% \end{equation}
% where $n$ is the number of facts in the generated story; $s_i$ is the importance score of $i$-th fact derived from the story generation algorithm, and $a_i$ is the area $i$-th fact occupied. With $f_s$, we expect that facts with higher scores would involve larger areas to attract enough attention from readers for they bring more information.

% Here we denote the layout of fact sheet with $n$ facts as $C = \{C_1, C_2, \cdots, C_k\}$, where $k$ is the number of rows in the fact sheet. Formally, $f_d$ is calculated as follows:
% \begin{equation}
% f_d = f_d^{inter} - f_d^{intra}
% \label{eq:opti_layout}
% \end{equation}
% \begin{equation}
% f_d^{inter} = \frac{\sum_{1 \leq j < |C|} d(C_j, C_j+1)}{|C|-1}
% \label{eq:opti_inter}
% \end{equation}
% \begin{equation}
% f_d^{intra} = \frac{\sum_{C_j \in C} \sum_{1 \leq i < |C_i|} fact\_distance(x_i, x_{i+1})} {n - |C|}
% \label{eq:opti_intra}
% \end{equation}
% where $fact\_distance$ measures the distance between two facts. To obtain it, we first calculate the similarity between two facts as described in Sec.4.3 and then minus it from one, indicating low similarities lead to high distances. As for the distance between two rows, we identify it as the distance between two adjacent facts connecting rows. Finally, $f_d$ is derived by subtracting $f_d^{intra}$, the average distance inside rows, from $f_d^{inter}$, the average distance between rows. With higher value, $f_d$ represents a more compact layout of a fact sheet in terms of the logic relations among facts through the generated story.


% \subsection{Interactions}
% % Describe the interactions of the system.

% \name provides a set of interaction methods to support the data story generation, fact exploration, story visualization and publishing to the public web.

% {\bf Data story generation.} \name allows users to fine-tune several details of the story in the story configuration panel within the storyline view. For the length of the story generated by \name, the chart diversity for each fact type and the time limitation of generation, users can drag the sliders of each parameter to pick a specific value from the given range. As for the reward preference for the generation, user can drag the circle $S$ which presents the story in the reward panel, to a position where distances between the story circle and three aspect nodes capture the relevant weights accordingly. After all parameters settled, users can click the ``Generate Story" button and wait for the story from \name in a few seconds. With the generated story, \name allows users to add a new fact piece or remove current fact pieces by clicking buttons, or re-order the fact pieces by simple drag-and-drop interaction in the story pieces panel. Editing the fact description is also enabled in the story pieces panel. All actions will apply in all the other views accordingly to reduce repetitive modification. 

% {\bf Modifying data fact.} The fact view enables users to customize this fact by changing the configuration. 
% Fact view provides selectors for \textit{fact type}, \textit{visualization}, \textit{measure},\textit{subspace}, \textit{group-by}, and \textit{focus}. When changing these configuration items, the current fact will be modified in real time. 

% {\bf Choosing visualization form and publishing.} 
% \name allows user to switch between all the visualization forms mentioned in~\ref{StoryView} in the story visualization view.
% By clicking the ``share" button, \name can automatically generate an online access link and a code snippet that can be embedded in other web pages for the generated data story represented in its current visualization form. When the user clicks the copy button, the online link or the code snippet will be copied accordingly. If others visit the link, they can access this data story. As for the generated 
% code snippet, user can easily embed this data story into his own web page by inserting the snippet into it.

==> sections-back/6-evaluation.tex <==
\section{Evaluation}
The evaluation of \name system consists of two parts, which respectively estimate the quality of the generated story logic and the visual data story content.


We evaluate \name via two controlled experiments to evaluate the generate logic and case study with 10 expert users followed by a series of expert interviews to collect their feedback.

\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{figures/case23.png}
  \vspace{-1.5em}
  \caption{Two alternative visualization modes, (a)\swiper mode and (b) \factsheet mode, that are developed to facilitate the story exploration, sharing and communication via mobile phones and printouts.} 
  \label{fig:vmodes}
  \vspace{-1em}
\end{figure*}

\subsection{Evaluation of the Generated Logic}
Two controlled experiments were performed to evaluate the generated story logic. The first one is designed to compares the logic generated by users and 

In the first experiment, we first randomized the orders of a set of data facts in a visual data story generated by \name and then asked a group of users to restore the order of the data facts based on their own observations and understandings of the data facts. Finally, we checked the consistency of the human generated logic orders and the logic order produced by \name. In this experiment, we recruited 20 participants (17 female) aged from 22 to 30 (mean 26). 11 of them had data analysis experiences and 14 of them had some basic knowledge about data visualization. 3 participants have experience in storytelling and 16 are with the skill of design. Participants took 19.5 minutes in average ($SD=10$) to finish the study.


\subsubsection{User Study \uppercase\expandafter{\romannumeral1}}
The first study evaluates the logicality of the data stories of \name by comparing the orders of facts from \name and human.

\textbf{Hypotheses} 
As we apply a logic-oriented MCTS to explore the space of the input data and generate data facts as a data story, we hypothesize that:
\begin{enumerate}
\itemsep -1mm
\item[{\bf H1}] The logic order of facts in the story generated by \name would strongly correlated with users' logical reasoning.
\end{enumerate}

\textbf{Procedure and Task} We collected three datasets in different topics to generate data stories for the study. \textit{CarSales} dataset(275 rows, 4 columns) describes the sales of different automobile brands from 2007 to 2011; \textit{COVID-19} dataset(903 rows, 6 columns) provides epidemic data around the world from Mar. 1, 2020 to Mar. 21, 2020, recording the number of infections, deaths and cures everyday; \textit{Startup Failures} dataset(1234 rows, 6 columns) reports the situation of companies that died through the tide of the new economy in China from 2010 to 2019, showing these companies' industry information, fund status they ended up with, reasons for failure, etc. For each dataset, we uploaded it to \name and generated 4 stories with length 6, then shuffled the order of each story. 

In the study, we presented brief introduction of each dataset before the questions. For each question, participants were asked to re-arrange the facts from an out-of-order story based on the information from charts and descriptions, to form a logical and reasonable story. After answering all 12 questions of re-ordering, participants were asked to write down their judgement and their personal information. 

\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{figures/userstudy1.png}
  \vspace{-2em}
  \caption{The evaluation results of the story logic: (a) the average Kendall's $\tau_b$ values and standard errors on each dataset; (b) the average Kendall's $\tau_b$ values and standard errors of Human and \name; (c) the means and standard errors of rates on logic of DataShot and \name by participants using a 5-point Likert scale.} 
  \label{fig:userstudy_tau}
  \vspace{-1.7em}
\end{figure}

\textbf{Results}
To measure the correspondence between the rankings of \name and of participants, we used Kendall's $\tau_b$ correlation~\cite{kendall1945treatment}  for evaluation, with value lies between -1(reversed order) and 1(original order). First we collected the participant scores of the Kendall's $\tau_b$ on the orderings between participants and \name and then averaged them on each dataset, as shown in Fig.~\ref{fig:userstudy_tau}(a). The results indicate that there exists some correlation between two rankings, especially in the latter two datasets, which are more familiar to the participants.   

To understand whether \name really perceives logic and generate meaningful stories, we invited an expert who knows much about the three datasets to assign reasonable orders of the facts of each story. Then we obtained the Kendall's $\tau_b$ correlation between participants' rankings and expert's rankings on 12 questions, marked as \textit{Human}, and the Kendall's $\tau_b$ correlation between \name's rankings and expert's rankings on 12 questions, marked as \textit{\name}. We conducted an unpaired t-test to examine the differences on the $\tau_b$ scores of two groups. The result showed in Fig.~\ref{fig:userstudy_tau}(b) indicates that there is no significant difference ($t(22)=.097, p=.92$) of participants($M=.50, SD=.13$) and \name($M=.55, SD=.17$) when comparing both of their rankings with that of the expert. Hence \textbf{H1} is accepted.

When asked about the criteria of a logical story, the answers can be summarized into four aspects. 
% 内容连贯性
First, most of the participants valued the consistency of stories. \textit{``I would pay attention to the key words in the facts, and place those with similar key words together"}, one participants said. Since our stories were backed up by data, some participants arranged the facts by tracking the relevant data scopes as well. 
% 篇章结构
Secondly, participants would try to organize data facts using common discourse relations. Among the answers(9 of 20), the overall-detail structure of stories was mentioned most frequently, with which the story gives the whole picture in the beginning, followed by a series of details. 
% 语义理解
Also, participants would interpret the semantic contents of each fact. one commented that \textit{``I assigned the orders through the emotions from negative to positive for the COVID-19 dataset, first reporting the number of infections, then deaths and cures."} while another said that \textit{``I followed the chronological order and put facts depicting infections of COVID-19 ahead of those with deaths situation."} 
% 可视化形式
Particularly, since \name presents data stories with visualizations, some participants(5 of 20) mentioned that they would take the visualizations into account. One commented that one of his judgements was \textit{``the correlation of types of charts in each fact"}.

\subsubsection{User Study \uppercase\expandafter{\romannumeral2}}
To further evaluate the quality of the output of \name, we conducted the second user study to validate whether the data stories generated by our approach would be more logical and reasonable than existing work. For comparison, we choose DataShot\cite{wang2019datashot} as a baseline, which automatically generates ``random facts" sheet from the tabular data. 

\textbf{Hypotheses} 
% We hypothesize that, by using logic-oriented MCTS, Calliope's fact order would strongly correlated with users' order.
As the facts in our stories follow a logical order and are displayed sequentially in all visualization modes, we hypothesize that:
% As the facts in our generated visualization are in a logical order, we hypothesize that:
\begin{enumerate}
\itemsep -1mm
\item[{\bf H2}] The visual data story generated by \name would be better for reading than the story with facts in random order under the same topic significantly.
\end{enumerate}

\textbf{Participants} In this study, we invited 20 participants (14 female) whose ages range from 23 to 30 (mean: 25). All the participants are students majoring in design. 13 of them have the experience in designing infographic posters. They took an average of 13 minutes ($SD=12$) to complete this study.

\textbf{Procedure and Task} Our study followed a 2 (visualization tool) $\times$ 3 (dataset) mixed design. We collected the three datasets presented in DataShot and uploaded them to \name to generate stories in the \factsheet mode. After the processing, we got 6 factsheets, including 3 of them collected from the paper of DataShot and the other 3 generated from \name. To avoid other factors that interfere with the study, we unified the design style for the factsheets from both visualization tools. We also marked the sequential number for all facts in each factsheet to guide participants. Finally, we randomized the order of the 6 factsheets in each questionnaire.

Each participant performed 6 trials in the questionnaire. In each trail, participants were shown one factsheet and asked to read it following the sequential order from left to right, top to bottom. After each trail, they rated the logic of the factsheet in a 5-point Likert scale ranging from ``Very Unclear" to ``Very Clear".

\textbf{Results} We analyzed a total of 120 user ratings and conducted unpaired t test between DataShot and \name. The result (Fig.~\ref{fig:userstudy_tau}(c)) shows that there is a significant difference ($t(118)=3.99, p<.01$) between the rating of DataShot($M=3.02, SD=.95$) and \name($M=3.72, SD=.98$), which means that stories generated by \name have clearer logic than random facts stories for reading and comprehension. Therefore \textbf{H2} is accepted. 

\subsection{Case Studies and Expert Interview}
% Show three example stories generated by Callipoe based on the three datasets that we have. 

To evaluate the utility of our system, we conducted in-depth interviews with ten experts. Due to the application fields of the system, we chose experts from three relevant areas, including 4 professional data journalists, 3 data analysts in BI department, and 3 visualization researchers. In the following section, these 10 participants are denoted as \textbf{P1}, \textbf{P2}, ..., \textbf{P10}, where \textbf{P1-P4} are data journalists, \textbf{P5-P7} are data analysts, and \textbf{P8-P10} are visualization researchers.

\textbf{Interview methodology} 
The interview was started with a 10-minute system introduction. We introduced the system interface and each module to the interviewees. 
Then all the participants were asked to explore our system freely and generate a high quality data story with a provided dataset in 15-20 minutes. During the exploration process, if participants have any questions with \name, we'll provide hints to them promptly. After finishing exploring and completing a data story, the user was asked to use the sharing feature to generate a link as a delivered work.
Then we conducted a brief interview with the user, including the following three aspects: the generated data story, visual and interaction design and the overall system. 
At the end of the interview, the participants were asked to fill out a questionnaire to assess these three aspects using a 5-point Likert scale.
On average, each of the interviews last approximately one hour.

\textbf{Case Studies}
We collected all visual data stories authored by participants. Here we present three of them with different spreadsheets, including CarSales, COVID-19, and Startup Failures.

\textit{CarSales.} \textbf{P7} (data analyst, male, 34) generated and authored this story about CarSales, which is shown in Fig.~\ref{fig:vmodes}(a). During the whole authoring process, he acknowledged that the generated story is well structured which can be easily understood and provided an overview of the dataset. Thus, he used the generated story as backbone and edited facts to convey his insights about this data. The final story is start with the sales trend from 2007 to 2011. He thought the financial crisis is to blame for this decreasing trend. Then the story shows the rank of sales for each brand and the top 1 Ford accounts for 25.04\% of the total sales. After that, it displays the rank of sales for different vehicle models and the comparison between top 1 (SUV) and top 3 (Subcompact). In the end of the story, P7 indicated that the sales of Subcompact model is the only one not recovered after the financial crisis. After finishing the story, he shared it in \swiper mode which he thought is the best way to spread via phones quickly. 

\textit{COVID-19.} This story is generated and authored by \textbf{P4} (data journalist, female, 25), which is shown in Fig.~\ref{fig:teaser}. P4 is an experienced data journalist. Because of her daily work needing the cooperation with designers and engineers, she appreciated the effectiveness of this system that can let her create data news on her own. After the story generation, she use the data story editor to reorder facts to ensure the attractiveness of the story based on her background knowledge. The story first presents the distribution of death cases in the provinces of China during March and points out that the maximum is 42 on March 2. Then it displays the distribution of death cases geographically, followed by the detail data in Hubei. After that, the story is concluded with the total death and recovered cases in March, indicating that China has turned for the better. She decided to represent the story in the \storyline mode, which can be embedded into websites for news reports easily and read in web browsers.
% Then it displays the increasing trend of confirmed cases in the whole world. After that, it shows the tendency of death cases and recovered cases one after another.
% For the purpose of propagation, she decided to use \storyline mode
% which she thought is the best form to present and share with the public instantly. 

\textit{Startup Failures.} \textbf{P10} (visualization researcher, female, 29) was interested in the spreadsheet about startup failures in the past 10 years. She has no background information about this data before. Instead of the data exploration, she started with the story generation in the \name system. 
This generated story begins with the trend and distribution of failed startups in terms of time and space respectively, then represents the survival time ranking of failed startups in each industry and the situation of failed startups in each fund status. An outlier is also detected that no-funding is abnormal among all fund statuses. At the end of the story it shows the distribution of failure reasons of startups. After viewing the initial generated story, she pointed out that the logic and statement of generated story is very clear. Then she checked the schema of the data table and she found the generated story covers all aspects of the data. Thus she felt satisfied with the story without making any significant changes and only tried to adjust the visualization of the facts. Finally, she chose to print the story in the \factsheet mode as shown in Fig.~\ref{fig:vmodes}(b). 

\textbf{Participant Feedback} 
After the interview, we summarized all the participants' feedback and collated the results of user ratings of \name.
Fig.~\ref{fig:interview} shows the results of a 5-point Likert scale, which express how much the users agree or disagree with 8 standards on 3 aspects of our system. Generally speaking, all the expert users gave promising and positive feedback on \name.

\begin{figure}[tbh]
  \centering
  \includegraphics[width=\linewidth]{figures/interview.png}
  \vspace{-1.5em}
  \caption{The interview ratings of \name on a 5-point Likert scale.} 
  \label{fig:interview}
  \vspace{-0.5em}
\end{figure}

\textit{\textbf{The generated data story.}} 
% 是否有效传达数据信息
All the experts agreed that the data stories generated by \name can effectively convey the necessary information in the data. 
\textbf{P10} commented, \textit{``Each part of the story has the information that I want to present, and the story has both the overall content and the details. It's amazing!"}. 
% 系统是否能帮助我们探索数据
Experts commented regarding the data exploration that, \textit{``This system can effectively help users explore data in order to discover intriguing data facts"}(\textbf{P3}), and \textit{``The system automatically generates structured framework of data stories about the dataset, helping users to explore and understand the data easily"}(\textbf{P7}).
% 生成故事的逻辑
Meanwhile, participants commented on the logic of the generated story, \textit{``The logic of the generated story is very clear, especially when the logicality attribute in the reward panel was adjusted to a larger value"} (\textbf{P9}), and
\textit{``The logical order of the generated story can help the readers get to the point"}(\textbf{P1}).
% 故事片段的展现形式
Moreover, experts also reported that the current presentation of data facts is meaningful and easy to understand.
\textbf{P5} commented, \textit{``Instead of presenting multi-dimensional data in complex visualizations, the system arranges the appropriate dimensions and measures, and uses a series of simple visualizations to make the generated story easier to understand." }

\textit{\textbf{Visual and interaction design.}}
All experts provided positive comments on the visual and interaction design of \name.
% 3 种可视化形式
Regarding the 3 visual forms of the data story, expert users acknowledged that these 3 visual forms are very useful and can be selected for different scenarios. 
Experts commented, \textit{``Each fact in the \factsheet mode is sized according to how important it is. Therefore, it makes sense that this layout allows people to see relatively important information of the data story at a glance. It's also very nice that the \factsheet can be printed as a PDF"}(\textbf{P3}); 
\textit{``The \swiper mode shows a fact per page, which is suitable for mobile devices"}(\textbf{P9});
\textit{``The \storyline mode is a great form for presenting stories in web pages"}(\textbf{P7}).
% storyline view and fact view
As for the storyline view and the fact view, \textbf{P9} appreciated the interaction between these two views. He commented, \textit{``I can roughly explore the whole data story through the storyline view, and then further explore the data details on each of its fields of the selected fact through the fact view."}
% 增加、删除、重排
\textbf{P3} also expressed her thoughts in that, `\textit{`The storyline view enable me to add, delete, reorder and modify generated data facts, which is really convenient for me to make a data story on my preference"}
% reward panel 调整故事的3个属性
At the same time, two experts(\textbf{P3} and \textbf{P9}) mentioned that the adjustment of reward configuration can help users with different needs to generate stories with different emphasis, \textit{``For example, data journalists like me may focus more on the logicality of a data story, while data analysts may prefer integrity because they may want to cover as much data as possible"}(\textbf{P3}).
% 修改文本
% Experts especially appreciate the feature of text editing, \textit{``Text editing function can help me freely adjust the text of the story"}(\textbf{P2}).

\textit{\textbf{The overall system.}}
These 10 experts all gave an overall assessment of \name from the perspective of their areas of expertise.
% data journalist
\textbf{P1}, a data journalist with four years' experience, commented that this system can help users generate stories quickly and intelligently, compared to traditional journalism, which uses templates to draw charts. 
\textbf{P2} also appreciated the effectiveness of \name. she commented, \textit{``This system is very useful and gives a lot of effective advice, especially for those who have no experience in data visualization or data journalism."}
Another data journalist \textbf{P4} said the system enable users to quickly create graphics for some easy-to-read articles with little interaction, thus there is no need for the designers to typesetting. She also commented that charts provided in \name are commonly used in journalism, such as line charts, bar charts, pie charts, etc.
% data analysts
The data journalist offered insights of our system from a news perspective, while data analysts came up with insights from the perspective of data analysis.
\textbf{P7} commented, \textit{``With this system, analysts can quickly generate stories that help quickly summarize the information of the data without much exploration or insight. It is really convenient in simple application scenarios."}
% visualization experts
In addition, data visualization experts also put forward their own views.
\textbf{P9} commented, \textit{``The system lays out the overall story frame of a dataset, giving us a direction on how to create a data story. It is worth mentioning that the visual design is also very good."}
\textbf{P10} said, \textit{``The overall system is very useful, especially for people who are not professional in data visualization."}


\textbf{Discussions}
In spite of the positive feedback mentioned above, some suggestions for our system were also put forward, which can be summarized in the following aspects:
\begin{itemize}[leftmargin=10pt,topsep=2pt]
\itemsep -.5mm
    \item {\textbf{Story optimization.}} 
    Both \textbf{P2} and \textbf{P9} said that the automatic-generated text may be suitable for Simple application scenarios or initial story exploration. However, the formal scenarios, such as professional news, have high requirements of expression. They suggested the statement of the story can be more diverse and vivid. 
    Journalists are more concerned about the specific cases behind the data, hoping to dig deeper into the information behind the data.
    Meanwhile, data analysts also pointed out that the data story just describe the data fact without further insight which can guide users on how to take actions.
    These concerns indicate the gap between generated and real-world data stories. Since \name provides editing functions, users can further optimize the generated stories to meet their needs on various aspects. 
    
    \item {\textbf{Semantic understanding.}} Three experts (\textbf{P3}, \textbf{P6}, \textbf{P7}) pointed out that the generated data stories are lack of semantic understanding and common sense to build bridges between information. For example, in the news about COVID-19, the number of confirmed cases is usually depicted before the number of deaths and cures. However, our system does not have this background knowledge. We acknowledge it as the limitation of the current system. Spreadsheets in the real world are usually relevant to some domain knowledge, which has significant impact on the story structure. We think it is a promising direction for future work.
    
    \item {\textbf{Visualization.}}
    \textbf{P2}, \textbf{P3} and \textbf{P4} all suggested that the system should provide the ability to customize charts(such as changing color, transparency, axis labels, etc.) and provide more visual designs for users to choose. Regarding the \factsheet mode, 3 of the experts suggested that the reading order of the data facts should be more clear. Moreover, \textbf{P10} suggested, \textit{``I'd appreciate it if there was a visualization form of slides, which can be helpful when I need to prepare a presentation."} As future work, we plan to integrate more charts and layouts to enrich our system.
\end{itemize}

Overall, \name is appreciated by these ten experts. These interviews also pointed out the next steps of the system.

==> sections-back/algorithm-back.tex <==
Generally, the algorithm, as shown in Algorithm~\ref{alg:generation}, takes a spreadsheet $\mathcal{D}$, i.e., a data table, and the desired story length $\mathcal{L}$ as the inputs and generates a story  $\mathcal{S} = \{f_1,\cdots,f_n\}$ automatically. Specifically, it first randomly generates a set of initial facts in three fact types, i.e., value, trend, and categorization, that are most frequently used as a starting point in a data story according to our preliminary survey as shown in  Fig.~\ref{fig:statistic}(b) (line 1). The most important fact, denoted as $f_0$, is selected into the story and used as the root of a search tree (line 2). In the next, the algorithm predicts a set of logic relations $\mathcal{R}$ that are likely to occur after the last fact $f$ in the current story (line 3). The prediction is achieved by a Markov chain model~\cite{}, which is trained based on a set of fact-relation pairs labeled during our preliminary survey as summarized in Table.~\ref{tab:logic}. After that, the algorithm expands
$f$ by randomly creating a set of data facts $\mathcal{F}$ that are logically relevant to it based on a relation $r_i \in \mathcal{R}$. $r_i$ is randomly selected from $\mathcal{R}$ regarding to its occurrence probability estimated by the prediction model (line 6, 7). A reward function is used to estimate the quality of each fact in $\mathcal{F}$ in context of the current story. The fact $f_{i}$ with the largest reward score regarding to $r_i$ is identified as a local optima used to update the search tree though a back-propagation process (line 8, 9). The above steps (line 5 - 9) repeat until the computation exceed a time limitation that guarantees an efficient generation process ({\bf R2}).
Finally, the fact with the best reward score among all the facts generated based on all possible logic is added into the search tree as a child of $f_i$ and at the end of the story, which will be further explored and expanded in the next iteration. The algorithm stops until a desired story length is reached. In the next, we will describe the policy used for expanding a fact in a given logic and the reward function used for estimating the story quality.

\begin{algorithm}[htb]
    \label{alg:generation}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$\mathcal{D}, \mathcal{L}$}
    \Output{$\mathcal{S}$}
    % \KwResult{Write here the result }
    $f_0$ $\leftarrow$ Initialize($\mathcal{D}$)\;
    $\mathcal{S}$ $\leftarrow$ \{$f_0$\}\;
    \While{$|\mathcal{S}|$ \textless $\mathcal{L}$}{
    
        $\mathcal{R} \leftarrow LogicPredict(\mathcal{S})$\;
    
        \While{within time limitation}{
            $r_i$ $\leftarrow$ ProbabilisticRandomFetch($\mathcal{R}$)\;
            $\mathcal{F}$ $\leftarrow$ Expand($\mathcal{S}[|\mathcal{S}| - 1]$, $r_i$)\;
            $\{f_{i + 1},score\}$ $\leftarrow$ Reward($\mathcal{S}, \mathcal{F}$)\;
            BackPropagation($f_{i + 1}$, $r_i$, $score$)\;
        }
        $\mathcal{S} \leftarrow \mathcal{S} \cup \{f_{best}\}$\;
    }
    % $\mathcal{S} \leftarrow Aggregation(\mathcal{S})$\;
    \Return $\mathcal{S}$\;
    \caption{Data Story Generation}
\end{algorithm}

% full version for the algorithm implementation
\begin{algorithm}[htb]
    \label{alg:generation}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$\mathcal{D}, \mathcal{L}$}
    \Output{$\mathcal{S} = \{f_1, \cdots, f_n\}$}
    % \KwResult{Write here the result }
    $f_0$ $\leftarrow$ Initialize($\mathcal{D}$);
    $\mathcal{T}$ $\leftarrow$ \{$f_0$\};
    $\mathcal{S}$ $\leftarrow$ \{\}\;
    \While{$|\mathcal{S}|$ \textless $\mathcal{L}$}{
        \tcc{1.\selection}
        $f_i \leftarrow select(\mathcal{T})$\; 
        
        \tcc{2.\expansion}
        $\mathcal{R} \leftarrow LogicPredict(f_i)$\;
        $\mathcal{F}$ $\leftarrow$ Expand($f_i$, $\mathcal{R}$)\; 
        
        \tcc{3.\simulation}
        $\mathcal{T}_s \leftarrow \{f_i\}$\;
        \While{within time limitation}{
            
            $\Delta \leftarrow$ Reward($\mathcal{T}_s, \mathcal{F}$)\;
            
            $\Delta^* \leftarrow$ BackPropagation($\mathcal{T}_s, \Delta$)\;
            
            $f_i \leftarrow select(\mathcal{T}_s)$\;
            $\mathcal{R} \leftarrow LogicPredict(f_i)$\;
            $\mathcal{F}$ $\leftarrow$ Expand($f_i$, $\mathcal{R}$)\; 
        }
        \tcc{4.\backprop}
        BackPropagation($\mathcal{T}, \Delta^*$)\;
        
        $\mathcal{S} \leftarrow \mathcal{P}_{best}$\;
    }
    % $\mathcal{S} \leftarrow Aggregation(\mathcal{S})$\;
    \Return $\mathcal{S}$\;
    \caption{Data Story Generation}
\end{algorithm}

==> sections-back/narrativelogic.tex <==
\begin{table}[tb]
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\caption{The narrative logic frequently used after each fact type.}
\label{tab:logic}
\centering
\small
\def\arraystretch{1.5}
\setlength\leftskip{0pt plus 1 fil minus \marginparwidth}
\begin{tabular}{ccccccc}
\toprule
\rotatebox{0}{Fact Types}         & \rotatebox{70}{Similarity(\%)} & \rotatebox{70}{Temporal(\%)} & \rotatebox{70}{Contrast(\%)} & \rotatebox{70}{Cause-effect(\%)} & \rotatebox{70}{Elaboration(\%)} & \rotatebox{70}{Generalization(\%)} \\\midrule
Value          & \cellcolor[HTML]{6BAED6}35.9 & \cellcolor[HTML]{EFF3FF}8.9  & \cellcolor[HTML]{EFF3FF}9.7  & \cellcolor[HTML]{EFF3FF}4.2  & \cellcolor[HTML]{9ECAE1}26.8 & \cellcolor[HTML]{C6DBEF}14.5 \\
Difference     & \cellcolor[HTML]{6BAED6}34.5 & \cellcolor[HTML]{EFF3FF}6.7  & \cellcolor[HTML]{EFF3FF}7.1  & \cellcolor[HTML]{EFF3FF}5.8  & \cellcolor[HTML]{6BAED6}31.1 & \cellcolor[HTML]{C6DBEF}14.8 \\
Proportion     & \cellcolor[HTML]{4292C6}42.4 & \cellcolor[HTML]{EFF3FF}7.3  & \cellcolor[HTML]{EFF3FF}9.7  & \cellcolor[HTML]{EFF3FF}5.2  & \cellcolor[HTML]{9ECAE1}22.4 & \cellcolor[HTML]{C6DBEF}13.0 \\
Trend          & \cellcolor[HTML]{6BAED6}34.7 & \cellcolor[HTML]{EFF3FF}9.4  & \cellcolor[HTML]{EFF3FF}8.2  & \cellcolor[HTML]{EFF3FF}7.1  & \cellcolor[HTML]{9ECAE1}28.2 & \cellcolor[HTML]{C6DBEF}12.4 \\
Categorization & \cellcolor[HTML]{9ECAE1}27.9 & \cellcolor[HTML]{EFF3FF}3.4  & \cellcolor[HTML]{EFF3FF}9.8  & \cellcolor[HTML]{EFF3FF}3.4  & \cellcolor[HTML]{4292C6}47.5 & \cellcolor[HTML]{EFF3FF}7.8  \\
Distribution   & \cellcolor[HTML]{4292C6}41.7 & \cellcolor[HTML]{C6DBEF}12.1 & \cellcolor[HTML]{EFF3FF}7.3  & \cellcolor[HTML]{EFF3FF}4.4  & \cellcolor[HTML]{9ECAE1}22.3 & \cellcolor[HTML]{C6DBEF}12.1 \\
Rank           & \cellcolor[HTML]{6BAED6}32.1 & \cellcolor[HTML]{C6DBEF}11.7 & \cellcolor[HTML]{C6DBEF}11.7 & \cellcolor[HTML]{EFF3FF}6.6  & \cellcolor[HTML]{6BAED6}34.3 & \cellcolor[HTML]{EFF3FF}3.6  \\
Association    & \cellcolor[HTML]{6BAED6}31.0 & \cellcolor[HTML]{EFF3FF}5.6  & \cellcolor[HTML]{C6DBEF}15.1 & \cellcolor[HTML]{EFF3FF}7.1  & \cellcolor[HTML]{9ECAE1}26.2 & \cellcolor[HTML]{C6DBEF}15.1 \\
Extreme        & \cellcolor[HTML]{4292C6}40.7 & \cellcolor[HTML]{EFF3FF}5.6  & \cellcolor[HTML]{C6DBEF}11.1 & \cellcolor[HTML]{EFF3FF}3.7  & \cellcolor[HTML]{9ECAE1}25.9 & \cellcolor[HTML]{C6DBEF}13.0 \\
Outlier        & \cellcolor[HTML]{9ECAE1}20.0 & \cellcolor[HTML]{C6DBEF}10.0 & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{C6DBEF}10.0 & \cellcolor[HTML]{4292C6}40.0 & \cellcolor[HTML]{9ECAE1}20.0 
\\\bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

==> tables/4-relation.tex <==
\begin{table}[htb]
    \centering
    \label{table:relation}
    % \small
    \caption{The definition of 6 coherence relations}
    \begin{tabular}{ll}
    \toprule
    \textbf{Relation} & \textbf{Syntax} \\ \midrule
    Similarity & \{\{$f_i$\}\}. \{\{$f_{i+1}$\}\}. \\ 
    Temporal & \{\{$f_i$\}\}. After that, \{\{$f_{i+1}$\}\}. \\ 
    Contrast & \{\{$f_i$\}\}. However, \{\{$f_{i+1}$\}\}. \\ 
    Causality & \{\{$f_i$\}\}. The reason is \{\{$f_{i+1}$\}\}. \\ 
    Elaboration & \{\{$f_i$\}\}. Furthermore, \{\{$f_{i+1}$\}\}. \\ 
    Generalization & \{\{$f_i$\}\}. In general, \{\{$f_{i+1}$\}\}. \\ \bottomrule
    \end{tabular}
\end{table}

==> tables/datafacttable-backup.tex <==
\begin{table*}[t]
    \caption{Data Facts}
    \label{tab:fact_table}
    \small
    \def\arraystretch{1.2}
    \begin{tabular}{|l|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|l|p{7.7cm}|}
    \hline
    fact type & \multicolumn{1}{l|}{measure} & \multicolumn{1}{l|}{subspace} & \multicolumn{1}{l|}{breakdown} & \multicolumn{1}{l|}{ focus } & parameter & sentence template \\ \hline
    Value & O & O & X & X & derived value & The \{\{aggregate\}\} \{\{measure\}\} is \{\{parameter\}\} when \{\{subspace\}\}. \\ \hline
    Difference & O & O & O & O & difference value & \begin{tabular}[c]{@{}l@{}}The difference between \{\{focus{[}1{]}\}\} and \{\{focus{[}2{]}\}\} regarding to their \\ \{\{aggregate\}\} \{\{measure\}\} is \{\{parameter\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Proportion & O & O & O & O & percentage & \begin{tabular}[c]{@{}l@{}}The \{\{focus\}\} accounts for \{\{parameter\}\} of the \{\{aggregate\}\} \\ \{\{measure\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Trend & O & O & O & X & increasing/decreasing & \begin{tabular}[c]{@{}l@{}}The trend of \{\{aggregate\}\} \{\{measure\}\} over \{\{group-by\}\} is \\ \{\{parameter\}\} when \{\{subspace\}\}.\end{tabular} \\ \hline
    Categorization & X & O & O & X & number of categories & \begin{tabular}[c]{@{}l@{}}Given \{\{subspace\}\}, there are \{\{parameter\}\} \{\{group-by\}\}(s) \\ which are \{\{C\_1\}\}, \{\{C\_2\}\}, \{\{...\}\}, and \{\{C\_n\}\}.\end{tabular} \\ \hline
    Distribution & O & O & O & X & N/A & \begin{tabular}[c]{@{}l@{}}The distribution of the \{\{aggregate\}\} \{\{measure\}\} over different \\ \{\{group-by\}\}(s) shows an overview of the data when \{\{subspace\}\}.\end{tabular} \\ \hline
    Rank & O & O & O & O & N/A & \begin{tabular}[c]{@{}l@{}}In the \{\{aggregate\}\} \{\{measure\}\} ranking of different \{\{group-by\}\}(s), \\ the top three \{\{group-by\}\}(s) are \{\{focus{[}0{]}\}\}, \{\{focus{[}1{]}\}, \{\{focus{[}2{]}\}\},\\ when \{\{subspace\}\}.\end{tabular} \\ \hline
    Association & O & O & O & X & correlation value & \begin{tabular}[c]{@{}l@{}}The Pearson correlation between the \{\{measure{[}1{]}\}\} and the \\ \{\{measure{[}2{]}\}\} is \{\{parameter\}\} in case of \{\{subspace\}\}.\end{tabular} \\ \hline
    Extreme & O & O & O & O & \begin{tabular}[c]{@{}l@{}}0: max/min\\ 1: extreme value\end{tabular} & \begin{tabular}[c]{@{}l@{}}Given \{\{subspace\}\}, the \{\{parameter{[}0{]}\}\} value of the \{\{aggregate\}\} \\ \{\{measure\}\}is \{\{parameter{[}1{]}\}\} when \{\{group-by\}\} is \{\{focus\}\}.\end{tabular} \\ \hline
    Outlier & O & O & O & O & outlier value & \begin{tabular}[c]{@{}l@{}}The\{\{aggregate\}\} \{\{measure\}\} of \{\{focus\}\} is an outlier when compare \\ with that of other \{\{group-by\}\}(s) when \{\{subspace\}\}.\end{tabular} \\ \hline
    \end{tabular}
\end{table*}

==> tables/narrativelogicbackup.tex <==
\begin{table}[tb]
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\renewcommand{\arraystretch}{0.2}
\centering
\small
\def\arraystretch{1.5}
\setlength\leftskip{0pt plus 1 fil minus \marginparwidth}
\begin{tabular}{ccccccc}
\toprule
\rotatebox{0}{Fact Types}         & \rotatebox{0}{$r_s$} & \rotatebox{0}{$r_t$} & \rotatebox{0}{$r_c$} & \rotatebox{0}{$r_a$} & \rotatebox{0}{$r_e$} & \rotatebox{0}{$r_g$} \\\midrule
Value          & \cellcolor[HTML]{4292C6}45.6 & \cellcolor[HTML]{EFF3FF}8.9  & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{EFF3FF}4.2  & \cellcolor[HTML]{9ECAE1}26.8 & \cellcolor[HTML]{C6DBEF}14.5 \\
Difference     & \cellcolor[HTML]{4292C6}41.6 & \cellcolor[HTML]{EFF3FF}6.7  & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{EFF3FF}5.8  & \cellcolor[HTML]{6BAED6}31.1 & \cellcolor[HTML]{C6DBEF}14.8 \\
Proportion     & \cellcolor[HTML]{4292C6}52.1 & \cellcolor[HTML]{EFF3FF}7.3  & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{EFF3FF}5.2  & \cellcolor[HTML]{9ECAE1}22.4 & \cellcolor[HTML]{C6DBEF}13.0 \\
Trend          & \cellcolor[HTML]{6BAED6}34.7 & \cellcolor[HTML]{EFF3FF}9.4  & \cellcolor[HTML]{EFF3FF}8.2  & \cellcolor[HTML]{EFF3FF}7.1  & \cellcolor[HTML]{9ECAE1}28.2 & \cellcolor[HTML]{C6DBEF}12.4 \\
Categorization & \cellcolor[HTML]{9ECAE1}37.7 & \cellcolor[HTML]{EFF3FF}3.4  & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{EFF3FF}3.4  & \cellcolor[HTML]{4292C6}47.5 & \cellcolor[HTML]{EFF3FF}7.8  \\
Distribution   & \cellcolor[HTML]{4292C6}49.0 & \cellcolor[HTML]{C6DBEF}12.1 & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{EFF3FF}4.4  & \cellcolor[HTML]{9ECAE1}22.3 & \cellcolor[HTML]{C6DBEF}12.1 \\
Rank           & \cellcolor[HTML]{4292C6}43.8 & \cellcolor[HTML]{C6DBEF}11.7 & \cellcolor[HTML]{FFFFFF}0.0 & \cellcolor[HTML]{EFF3FF}6.6  & \cellcolor[HTML]{6BAED6}34.3 & \cellcolor[HTML]{EFF3FF}3.6  \\
Association    & \cellcolor[HTML]{6BAED6}31.0 & \cellcolor[HTML]{EFF3FF}5.6  & \cellcolor[HTML]{C6DBEF}15.1 & \cellcolor[HTML]{EFF3FF}7.1  & \cellcolor[HTML]{9ECAE1}26.2 & \cellcolor[HTML]{C6DBEF}15.1 \\
Extreme        & \cellcolor[HTML]{4292C6}51.8 & \cellcolor[HTML]{EFF3FF}5.6  & \cellcolor[HTML]{FFFFFF}0.0 & \cellcolor[HTML]{EFF3FF}3.7  & \cellcolor[HTML]{9ECAE1}25.9 & \cellcolor[HTML]{C6DBEF}13.0 \\
Outlier        & \cellcolor[HTML]{9ECAE1}20.0 & \cellcolor[HTML]{C6DBEF}10.0 & \cellcolor[HTML]{FFFFFF}0.0  & \cellcolor[HTML]{C6DBEF}10.0 & \cellcolor[HTML]{4292C6}40.0 & \cellcolor[HTML]{9ECAE1}20.0 
\\\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{The frequency of coherence relations, including similarity ($r_s$), temporal ($r_t$), contrast ($r_c$), causality ($r_a$), elaboration ($r_e$), and generalization ($r_g$) used after the 10 fact types.}
\label{tab:logic}
\vspace{-1em}
\end{table}
